The Bernstein-von Mises theorem for Semiparametric Mixtures

Semiparametric mixture models are parametric models with latent variables. They are defined kernel, $p_\theta(x | z)$, where z is the unknown latent variable, and $\theta$ is the parameter of interest. We assume that the latent variables are an i.i.d. sample from some mixing distribution $F$. A Bayesian would put a prior on the pair $(\theta, F)$. We prove consistency for these models in fair generality and then study efficiency. We first prove an abstract Semiparametric Bernstein-von Mises theorem, and then provide tools to verify the assumptions. We use these tools to study the efficiency for estimating $\theta$ in the frailty model and the errors in variables model in the case were we put a generic prior on $\theta$ and a species sampling process prior on $F$.

==> Frailty/LAN.tex <==
\subsection{LAN expansion for the Frailty model}
To prove the LAN expansion, we will use \Cref{Lem:LANByDonsker}.

\begin{lem}\label{lem:FrailtyModelLAN}
    Assume that $\theta_0 > 0$ and $F_0(z^2 + z^{-5}) < \infty$, then 
    \Cref{EqRemainders} holds for $P_{\theta_0, F_0}$.
\end{lem}

\begin{proof}
    We will verify each of the assumptions of \Cref{Lem:LANByDonsker}.
    \TODO{Least fav submodels etc}.
    \textbf{Step 1} Twice diff
    \TODO{write}
    \textbf{Step 2} Donsker
    \TODO{write}
    \textbf{Step 3} Integrable envelopes
    \TODO{write}
    \textbf{Step 4} Limits
    \TODO{write}
    \textbf{Conclude}
    \TODO{write}
\end{proof}
\TODO{Clean up using the new lemmas, which this a much smoother ride}.
The proof of this lemma takes some preparation.
This requires quite some preparation.

We will use \Cref{Lem:LANByDonsker} to conclude that \Cref{EqRemainders} holds for $P_{\theta_0, F_0}$.
\TODO{Ref} By consistency we can localise to any open neighbourhood of $\theta_0$ and $F_0$.
The efficient influence function is known and given by
\[
    \tilde\ell_{\theta_0, F}(x,y) = \frac{ \int \frac{1}{2} (x - \theta y) z^3 e^{-z( x + \theta y)} \dd F(z)}{\int \theta z^2 e^{-z( x + \theta y)} \dd F(z)}.
\]
As in \Cref{lem:FrailtyLeastFavSubmodel}, the least favourable submodel is given by 
\[
    F_t = F( B\left( 1 - \frac{t}{2 \theta} \right)^{-1} ).
\] 
In the notation of \Cref{Lem:LANByDonsker} and by using a change of variables, we find the perturbed likelihood:
\begin{align*}
    p_{\theta_t, F_t} &= \int z^2 ( \theta + t) e^{-z( x + (\theta + t) y)} \dd F_t(z) \\
       &= \int \left( z \left( 1 - \frac{t}{2 \theta} \right) \right)^2 ( \theta + t) e^{ - z \left( 1 - \frac{t}{2 \theta}\right) ( x + (\theta + t)y)} \dd F(z).
\end{align*}
We will use \Cref{lem:ExpressionsForGradiantHessian}.
Note that 
\begin{align*}
    h_\theta(x \given z) &= 2 \log(z) + \log(\theta) -z(x + \theta y).\\
    \phi_{t,\theta}(z) &= z\frac{1 - t}{2 \theta}.
\end{align*}
Thus, $h_{\theta + t} (x \given \phi_{t,\theta} (z))$ has gradient 

\TODO{Finish up}
This means that the first derivative is given by
    \[
        f' = \dot p_{\theta_t, F_t} = \int (a_1 + a_2 xz + a_3 yz) z^2 e^{-z( b_1 x + b_2 y) } \dd F(z)
    \]
    where $a_1, a_2, a_3, b_1, b_2$ are given by:
    \begin{align*}
           a_1 &= \frac{\left(t - 2\theta\right)\left(6 t \theta\right)}{3 \theta^3},
        && a_2 = \frac{\left(t - 2 \theta\right)^2 (t + \theta)}{8 \theta^3},
        && a_3 = \frac{ \left( t - 2 \theta\right)^2\left( \theta - 2t \right)(t + \theta)}{8 \theta^3},\\
           b_1 &= \frac{(2\theta - t)}{2 \theta} = 1 - \frac{t}{2 \theta},
        && b_2= \frac{(2\theta - t)(t + \theta)}{2 \theta} = \left( 1 - \frac{t}{2 \theta} \right)\left( \theta + t \right)
    \end{align*}
    Similarly, for the second derivative, we find
    \[
        f'' = \ddot p_{\theta_t, F_t} = \int (c_1 + c_2 xz + c_3 yz + c_4 x^2z^2 + c_5 xy z^2 + c_6 y^2 z^2) z^2 e^{-z(b_1x + b_2 y)} \dd F(z)
    \]
    where $b_1, b_2$ are as before and $c_1,\dots, c_6$ are given by
    \begin{align*}
           c_1 &= \frac{24 \theta^2 \left(t - \theta\right)}{16\theta^4}, 
        && c_2 = \frac{12 \theta (t - 2 \theta) t}{16 \theta^4}, 
        && c_3 = \frac{4 \theta (t - 2 \theta)( 7 t^2 - 4 t \theta - 2 \theta^2)}{16 \theta^4},\\
           c_4 &= \frac{ \left(t - 2 \theta\right)^2 \left( t + \theta\right)}{16 \theta^4},
        && c_5 = \frac{ \left(t - 2 \theta\right)^2 \left( t - \theta\right) \left( 2t - \theta \right) }{16 \theta^4},
        && c_6 = \frac{ \left(t - 2 \theta\right)^2 \left( t - \theta\right) \left( 2t - \theta \right)^2}{ 16 \theta^4}\\
    \end{align*}
    By now plugging in these expressions we find the first and second derivative of $\log p_{\theta_t, F_t}$. The first derivative is given by 
    \begin{align*}
        \frac{f'}{f} = \frac{\partial}{\partial t} \ell(t; \theta, F) &= 
        \frac{
            \int  (a'_1 + a'_2 x z + a'_3 yz)z^2 e^{-z( b_1 x + b_2 y)} \dd F(z)
        }{
            \int z^2 e^{-z( b_1 x + b_2 y)} \dd F(z)
        }
    \end{align*}
    where $b_1$ and $b_2$ are given as before and $a'_1, a'_2, a'_3$ are given as $a'_i = \frac{4 \theta^2 a_i}{\left(\theta + t \right)\left(2 \theta - t \right)^2}$.

    While for the second derivative we first compute $\frac{f''}{f}$.
    \begin{align*}
        \frac{f''}{f}&= 
        \frac{
            \int  (c'_1 + c'_2 x z + c'_3 yz + c_4 x^2 z^2 + c_5 xyz^2 + c_6 y^2z^2)z^2 e^{-z( b_1 x + b_2 y)} \dd F(z)
        }{
            \int z^2 e^{-z( b_1 x + b_2 y)} \dd F(z)
        }
    \end{align*}
    where $b_1, b_2$ are given as before, and $c_i' = \frac{ 4 \theta^2 c_i}{ \left(\theta + t \right) \left(2 \theta - t \right)^2}$.
    We can then finally plug this in to get 
    \[
        \frac{\partial^2}{\partial t^2} \ell(t; \theta, F) = \frac{f''}{f} - \left( \frac{f'}{f} \right)^2.
    \]

    Before we proceed, we introduce a useful helper function. 
    \[
        h_F(s) = \frac{ \int z^{m+2} e^{-zs} \dd F(z)}{ \int z^2 e^{-zs} \dd F(z) }.
    \]
    By applying \TODO{Cite Lemma L.23 Pfzanzagl} repeatedly, it follows that there exists constants and a weak neighbourhood $V$ of $F_0$ such that
    \[
        \sup_{F \in V} h_F(s) \leq \begin{cases} C_m s^{-m} | \log s |^m & \text{if } s < \frac{1}{2} \\ C & \text{if } s \geq \frac{1}{2}. \end{cases}
    \]

    Furthermore, observe that
    \[
        \frac{u^k v^l}{\left( b_1 u + b_2 v \right)^{k+l}}
    \]
    is totally bounded.
    
    This then allows us to provide uniform bounds on $\frac{f'}{f}$ and $\frac{f''}{f}$:
    

    \begin{align*}
        \sup_{ \theta \in U} \sup_{F \in V} \frac{ f'_{\theta, F}}{ f_{\theta, F}} & \lesssim \log( X) + \log( \theta_0 Y) + |X| + |Y| \\
        \sup_{ \theta \in U} \sup_{F \in V} \frac{ f''_{\theta, F}}{ f_{\theta, F}} & \lesssim \log(X)^2 + \log(\theta_0 Y)^2 + |X|^2 + |Y|^2
    \end{align*}
    Note that $\log(X)^2, \log(Y)^2, |X|^2$ and $|Y|^2$ all are $P_{\theta_0, F_0}$ integrable.
    
    Finally, this allows us to prove \Cref{lem:FrailtyModelLAN}
\begin{proof}
    \textbf{Twice continuous differentiability of the log likelihood}
    This follows from \Cref{remark:TwiceDiff}.
    \textbf{Verification of \Cref{Lem:LANByDonsker} a:}
    

    
    To apply \Cref{Lem:LANByDonsker} (a), we need to show that the class of first derivatives is Donsker and that $P_0 \| \dot\ell(t_n/\sqrt{n}; \theta_n, F_n) - \tilde\ell_0 \|^2 \rightarrow 0$.
    We will verify the Donsker condition first, and the limit will be shown using the dominated convergence theorem.



    \textbf{The derivatives of the perturbed log likelihood form a Donsker class}

    By~\cite[Lemma 25.87]{vandervaartAsymptoticStatistics1998} we see that this defines a Donsker class when $\theta$ is contained in a compact set and $F$ is in a suitable open neighbourhood of $F_0$. 
    By consistency, we can restrict to these sets, so this class is indeed Donsker.
    
    \textbf{The $L^2$ convergence to the efficient score function}

    First note that $\tilde\ell(\theta, F) = \dot\ell (0; \theta, F)$. 
    So we want to show that
    \[
        P_{\theta_0, F_0} \| \dot\ell( \frac{t_n}{\sqrt{n}}; \theta_n, F_n) - \dot\ell(0; \theta_0, F_0) \|^2 \rightarrow 0
    \]
    For this, first we show that this is true pointwise and that this is bounded, so we can apply the dominated convergence theorem.\\
    \textbf{Step a1: pointwise convergence}
    We want to show that
    \[
        \dot\ell\left( \frac{t_n}{\sqrt{n}}; \theta_n, F_n\right) - \dot\ell(0; \theta_0, F_0) \rightarrow 0.
    \]
    First note that
    \[
        \dot\ell\left( \frac{t_n}{\sqrt{n}}; \theta_n, F_n\right) = a_1 +  \frac{
            \int (a_2 x + a_3 y) z^3 e^{-z (b_1 x + b_2 y)} \dd F_n(z)
        }{
            \int z^2 e^{-z( b_1 x + b_2 y)} \dd F_n(z)
        }
    \]
    There exists a $C> 0$ such that $|a_1| \leq \frac{C}{\sqrt{n}}$. 
    Here we may assume that $\theta_n \rightarrow \theta_0$ and $F_n \rightarrow F_0$, by slowly shrinking our neighbourhoods.
    We will be using the formula for $\dot\ell(t; \theta, F)$ and plug in the values of $\frac{t_n}{\sqrt{n}}$, $\theta_n$ and $F_n$ respectively.
    If $\theta_n \rightarrow \theta_0$, and $t_n$ remains bounded, hence $\frac{t_n}{\sqrt{n}} \rightarrow 0$, we find that 
    \begin{align*}
        a_1 &\rightarrow 0,\quad 
        a_2 \rightarrow \frac{1}{2 \theta_0},\quad
        a_3 \rightarrow \frac{1}{2},\\
        b_1 &\rightarrow 1,\quad
        b_2 \rightarrow \theta_0.
    \end{align*}
    Note that for all $t, w > 0$
    \[
        \| w^l t^k e^{-tw} - e^{-(1 - \epsilon) tw} \| = w^l t^k e^{-tw} \| 1 - e^{\epsilon t} \| \leq w^l t^k e^{-tw} \left( \epsilon t w + \frac{ \left( \epsilon tw \right)^2}{2} \right) \lesssim \epsilon.
    \]

    Applying this to the terms in the denominator and applying the triangle inequality combined with the weak convergence of $F_n$ gives, for all $n$ large enough
    \begin{align*}
    \left\| \int z^2 e^{-z( b_1 x + b_2 y)} \dd F_n(z) \right.&-\left. \int z^2 e^{-z( x + \theta_0 y)} \dd F_0(z) \right\|\\ 
        &\leq \left\| \int z^2 e^{-z( b_1 x + b_2 y)} \dd F_n(z) - \int z^2 e^{-z( x + \theta_0 y)} \dd F_n(z)\right\| \\ 
        &+ \left\| \int z^2 e^{-z( x + \theta_0 y)} \dd F_n(z) -  \int z^2 e^{-z( x + \theta_0 y)} \dd F_0(z)\right\|\\
        &\leq 2 \epsilon
    \end{align*}
    Similarly for the numerator.
    Thus, for fixed $x,y$ we have convergence.

    \textbf{Step a2: Dominated convergence}

    By~\cite[Lemma 25.87]{vandervaartAsymptoticStatistics1998} there exists a square integrable envelope function $F (x,y)$. 
    By the triangle inequality 
    \[
        \|\dot\ell\left( \frac{t_n}{\sqrt{n}}; \theta_n, F_n\right) - \dot\ell(0; \theta_0, F_0) \| \leq 2 F(x,y) \forall \theta_n, F_n.
    \]
    Hence, we can apply the dominated convergence theorem, which implies the convergence in $L_2(P)$.

    \textbf{Verification of \Cref{Lem:LANByDonsker} part b:}
    
    Pointwise convergence given a fixed $x,y$ follows along the same arguments as in Step 1a.
    To see that this is a dominated function, we use the same argument as before.
    The final display is automatically satisfied for mixture models, see the discussion after the proof of \Cref{Lem:LANByDonsker}. 
\end{proof}



\begin{lem}\label{lem:uniformboundfrailtyefficientscore}
    Denote
    $f (a,b,x,y F) = \frac{
            \int (a_1 + a_2 x z + a_3 y z) z^2 e^{-z (b_1 x + b_2 y)} \dd F (z)
        }{
            \int z^2 e^{-z (b_1 x + b_2 y)} \dd F (z)
        }$
    Suppose that $a^{(n)} \rightarrow a^{(0)}$ and $b^{(n)} \rightarrow b^{(0)}$.
    Then
    \[
        \sup_{x,y, F} \| f(a^{(n)}, b^{(n)}, x, y, F) - f(a^{(0)}, b^{(0)}, x, y, F) \| \lesssim \|a^{(n)} - a^{(0)} \| + \| b^{(n)} - b^{(0)} \|
    \]
\end{lem}<++>
\begin{proof}
    First note that for $t > 0$.
        Applying this pointwise and integrating out shows that both integrals are, up to some constant independent of $x,y$ and $F$ within $\epsilon$ distance of each other.
    The final result follows.
\end{proof}



==> PartialLikelihood/PartialLikelihood.tex <==
\section{Partial Likelihood}
\TODO{Add references, get history right.}
See Cox 1975, Lindsay Partial likelihood.

Suppose that the kernel can be factored as
\[
    p_{\theta}(x \given z) = q_\theta(x)r_\theta(x \given z)
\]
\begin{definition}
    We call a likelihood factor $q_\theta(x)$ locally fully informative at $(\theta_0, F_0)$ if there exists a family $F_t$
    \[
        \int r_{\theta_0 + \alpha t}(x \given z) \dd F_t(z) = \int r_{\theta_0}(x, z) \dd F_0(z) \quad \textrm{for all } t \textrm{ small enough}.
    \]
\end{definition}

\subsection{Verifying the conditions}
\TODO{Prove LAN expansion}
\[
    p_{\theta,F}(x) = \int q_\theta(x \given z) r_\theta(x \given z) \dd F(z) = q_\theta(x) \int r_\theta(x \given z) \dd F(z).
\]
\begin{align*}
    p_{\theta + \alpha t, F_t}(x) &= \int p_{\theta + \alpha t}(x \given z) \dd F_t(z)\\
        &= \int q_{\theta + \alpha t}(x) r_{\theta + \alpha t}(x \given z) \dd F_t(z) \\
        &= q_{\theta + \alpha t}(x) \int r_{\theta + \alpha t}(x \given z) \dd F_t(z) \\
        &= q_{\theta + \alpha t}(x) \int r_{\theta}(x \given z) \dd F(z)
\end{align*}

\begin{lem}\label{lem:PartialLikelihoodChangeOfMeasure}
    Suppose that the prior density $h$ is continuously differentiable and non-zero in a neighbourhood $U$ of $\theta_0$. Suppose that the posterior is consistent for $\theta_0$. Then \Cref{EqChangeOfMeasure} holds.
\end{lem}
\begin{proof}
    By consistency, we can restrict the posterior to $U$.
    That is, it suffices to show that
    \[
        \frac{
            \int_U \prod_{i = 1}^n p_{\theta - \frac{t}{\sqrt{n}}, F_{-\frac{t}{\sqrt{n}}}(\theta, F)}(X_i) \dd \pi(\theta) \dd \Pi(F)
        }{
            \int \prod_{i = 1}^n p_{\theta, F}(X_i) \dd \pi(\theta) \dd \Pi(F)
        } \rightsquigarrow 1
    \]
    On $U$, by \Cref{lem:SmoothnessInH} we find that 
        \[
         \| \frac{h( \theta + \frac{t}{\sqrt{n}})}{h(\theta)} - 1 \| \leq \frac{C'_T}{\sqrt{n}}
    \]
    for all $\theta \in U$.
    Plugging this into the integral, combined with \Cref{lem:MoveRatioBoundIntoSum} and the expressions for $p_{\theta, F}$ and $p_{\theta - \frac{t}{\sqrt{n}}, F_{-\frac{t}{\sqrt{n}}}(\theta, F)}$ we find
    \begin{align*}
        &\frac{
            \int_U \prod_{i = 1}^n p_{\theta - \frac{t}{\sqrt{n}}, F_{-\frac{t}{\sqrt{n}}}(\theta, F)}(X_i) \dd \Pi(\theta, F)
        }{
            \int \prod_{i = 1}^n p_{\theta, F}(X_i) \dd \pi(\theta) \dd \Pi(F)
        }\\
        &= \frac{
            \int_U \prod_{i = 1}^n \left(q_{\theta - \frac{t}{\sqrt{n}}}(X_i)\int r_\theta(X_i \given z) \dd F(z)\right) \dd \pi(\theta) \dd \Pi(F)
        }{
            \int \prod_{i = 1}^n \left(q_{\theta}(X_i) \int r_\theta(X_i \given z) \dd F(z) \right) \dd \pi(\theta) \dd \Pi(F)
        }
    \end{align*}
\end{proof}


==> Supplements/Supplements.tex <==
\section{General supplementary material}
\TODO{check if needs to be removed}
\begin{lem}\label{lem:ErrorsInVarsPriorMassBound}
    Suppose that all assumptions of \Cref{lem:ErrorsInVarsPriorMassEps} are satisfied.
    Then
    \[
        \frac{e^{- c\sqrt{n} \log n}}{ \pi_t \otimes \textrm{DP}_t (B_{n,2} (p_{\theta, F}; p_{\theta_0, F_0}, \epsilon_n))} = o(e^{-2n \epsilon_n^2})
    \]
\end{lem}

\begin{proof}
    Pick $\epsilon_n = n^{-\alpha}$ for $a = \frac{1}{2}$.
    By \Cref{lem:ErrorsInVarsPriorMassEps} we know that
    \begin{align*}
        \pi_t \otimes \textrm{DP}_t(B_{n,2} (p_{\theta, F}; p_{\theta_0, F_0}, \epsilon_n)) &\leq= \pi \otimes \textrm{DP}_t( \textrm{KL} + V_2 \left( p_{\theta, F}; p_{\theta_0, F_0} \right) \leq \epsilon_n^2 )\\
            &\geq e^{-C \epsilon_n^{-\frac{1}{( 1 + \xi)}} \log( \epsilon_n^{-1})} \\
            &= e^{ - C' n^{\frac{\alpha}{(1 + \xi)}} \log n}
    \end{align*}
    Hence we want to show that
    \[
        e^{C n^{ \frac{\alpha}{2( 1 + \xi)}} \log n} e^{- c \sqrt{n} \log n} e^{2 n^{1 - 2 \alpha}} = o(1)
    \]
    It suffices to show that $\sqrt{n} \log(n)$ dominates both other terms.
    $n \epsilon_n^2 = n^{1 - 2 \alpha}$ is much smaller than $n^{1/2}\log(n)$ as soon as $\alpha \geq \frac{1}{4}$.
    For the choice $\alpha = \frac{1}{2}$ we get $n \epsilon_n^2 = 1$, and hence this term does not contribute.
    Now we need to show that $\sqrt{n} \log n$ also dominates $n^{\frac{\alpha}{(1 + \xi)}} \log (n)$.
    It suffices to show that $\frac{\alpha}{(1 + \xi)} < \frac{1}{2}$.
    This holds true as soon as $\alpha < \frac{1 + \xi}{2}$, which is true since $\xi > 0$.
\end{proof}



==> aad.tex <==
\catcode`\@=11 % allows @ to be used in control sequences in this format file


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{example}{Example}[section]
\newcommand{\prf}{\begin{proof}{Proof}}
%\renewcommand{\endproof}{\end{proof}}

\def\itemi{\item{(i)}}
\def\itemii{\item{(ii)}}
\def\itemiii{\item{(iii)}}
\def\itemiv{\item{(iv)}}
\def\itemv{\item{(v)}}
\def\itemvi{\item{(vi)}}


% Abbreviations
\def\A{{\cal A}} \def\a{{\alpha}}
\def\B{{\cal B}} \def\b{{\beta}}                        \def\BB{\mathbb{B}} \def\bB{{\bf B}}
\def\C{{\cal C}}                                        \def\CC{\mathbb{C}}
\def\D{{\cal D}} \def\d{{\delta}}     \def\gD{{\Delta}} \def\DD{\mathbb{D}}
                 \def\e{{\varepsilon}}                  \def\EE{\mathbb{E}} \def\bE{{\bf E}}
\def\F{{\cal F}} \def\f{{\phi}}                         \def\FF{\mathbb{F}}
\def\G{{\cal G}} \def\g{{\gamma}}                       \def\GG{\mathbb{G}}                           
\def\H{{\cal H}} \def\h{{\eta}}                         \def\HH{\mathbb{H}} \def\bH{{\bf H}}
\def\I{{\cal I}}                                        \def\II{\mathbb{I}} 
\def\J{{\cal J}}                                        \def\JJ{\mathbb{J}}              
\def\K{{\cal K}} \def\k{{\kappa}}                       \def\KK{\mathbb{K}}                              
\def\L{{\cal L}} \def\l{{\lambda}}    \def\gL{{\Lambda}}\def\LL{\mathbb{L}} \def\bL{{\bf L}}
\def\M{{\cal M}} \def\m{{\mu}}                          \def\MM{\mathbb{M}}
                 \def\n{{\nu}}                          \def\NN{\mathbb{N}}                              
\def\O{{\Omega}} \def\o{{\omega}}
\def\P{{\cal P}} \def\p{{\pi}}                          \def\PP{\mathbb{P}}
\def\Q{{\cal Q}} \def\q{{\theta}}                       \def\QQ{\mathbb{Q}}
\def\R{{\cal R}} \def\r{{\rho}}				\def\RR{\mathbb{R}}
                 \def\s{{\sigma}}     \def\S{{\Sigma}}  \def\SS{\mathbb{S}}
                 \def\t{{\tau}}       \def\T{{\Theta}}
\def\U{{\cal U}}					\def\UU{\mathbb{U}}
							\def\VV{\mathbb{V}}
\def\W{{\cal W}}                                        \def\WW{\mathbb{W}}
\def\X{{\cal X}} \def\x{{\xi}}				\def\XX{\mathbb{X}} \def\bX{{\bf X}}
\def\Y{{\cal Y}}					\def\YY{\mathbb{Y}} \def\bY{{\bf Y}}
\def\Z{{\cal Z}} \def\z{{\zeta}}                        \def\ZZ{\mathbb{Z}}


\def\sumin{{\sum_{i=1}^n}}
\def\sumjn{{\sum_{j=1}^n}}
\def\sumim{{\sum_{i=1}^m}}
\def\sumjm{{\sum_{j=1}^m}}
\def\sumik{{\sum_{i=1}^k}}
\def\sumjk{{\sum_{j=1}^k}}
\def\tsum{{\textstyle\sum\limits}}
\def\prodjn{{\prod_{j=1}^n}}
\def\prodin{{\prod_{i=1}^n}}
\def\prodim{{\prod_{i=1}^m}}
\def\prodjm{{\prod_{j=1}^m}}
\def\prodik{{\prod_{i=1}^k}}
\def\tprodik{\textstyle\prod_{i=1}^k\limits}
\def\tprod{{\textstyle\prod\limits}}
\def\prodm{\otimes} 
\def\prodmjn{{\bigotimes_{j=1}^n}}
\def\prodmin{{\bigotimes_{i=1}^n}}
\def\tprodmin{{\textstyle\bigotimes_{i=1}^n\limits}}
\def\tprodmjn{{\textstyle\bigotimes_{j=1}^n\limits}}
\def\tprodmim{{\textstyle\bigotimes_{i=1}^m\limits}}
\def\tprodmjm{{\textstyle\bigotimes_{j=1}^m\limits}}
\def\half{{\frac12}}
\def\thalf{{\textstyle\half}}
\def\tkwart{{\textstyle{\frac14}}}
\def\tint{{\textstyle\int\limits}}
\def\tbigcap{{\textstyle\bigcap\limits}}
\def\tbigcup{{\textstyle\bigcup\limits}}
\def\ra{\rightarrow}
\def\da{\downarrow}
\def\ua{\uparrow}
\def\dotfil{\leaders\hbox to 1em{\hss.\hss}\hfill}
\def\minqquad{\hskip-2em\relax}\def\minqqqquad{\hskip-4em\relax}
\def\qqqquad{\hskip4em\relax}\def\qqqqqquad{\hskip6em\relax}
\def\liminfsup{\mathop{\overline{\underline{\rm lim}}}}





% Mathematics
\def\hexnumber#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}
%\mathchardef\boxminus="3\hexnumber\msafam0C
%\mathchardef\lesssim="3\hexnumber\msafam2E
%\mathchardef\gtrsim="3\hexnumber\msafam26
%\mathchardef\rightsquigarrow="3\hexnumber\msafam20
\def\mypartial#1{\mathchoice{\partial\over\partial#1}{\partial/\partial#1}{}{}}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\entier#1{\lfloor#1\rfloor}
\def\BL{{\rm B\kern -0.5pt L}}
\def\UC{{\rm U\kern-0.5pt C}}
\def\linfty{\ell^\infty}
\def\simplex{{\rm S}}
\def\id{id}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}
\def\trace{{\rm trace }}
\def\diag{\mathop{\rm diag\,}\nolimits}
\def\lin{\mathop{\rm lin\,}\nolimits}
\def\closedlin{\overline{\lin}}
\def\tanh{\mathop{\rm tanh}\nolimits}
\def\arctanh{\mathop{\rm arctanh}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}
\def\loglog{\mathop{\rm loglog}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
%\def\interior{{\rm int}}
\def\interior{\mathaccent 23}
\def\closure#1{\overline{#1}}
\def\boundary{\mathop{\delta}\nolimits}
\def\closedhull{{\overline{\hull}}}
\def\closedconv{\closedhull}
\def\essinf{\mathop{\rm essinf}\limits}
\def\conv{\hull}
\def\hull{\mathop{\rm conv\ }\nolimits}
\def\diam{\mathop{\rm diam}\nolimits}
\def\ball{\mathop{\rm ball}\nolimits}
\def\closedball{\overline{\ball}}
\def\every{\hbox{ every }}
\def\forevery{\hbox{ for every }}
\def\OR{\hbox{ or }}
\def\implies{\hbox{ $\Rightarrow$ }}
\def\seilpmi{\hbox{ $\Leftarrow$ }}
\def\bydef{\buildrel {\rm def}\over =}
\def\qed{\ \vrule height4pt width4pt depth0pt}
\def\halmos{\ \vbox{\hrule\hbox{\vrule\vbox{\phantom{\vrule height4pt width4pt depth0pt}}\vrule}\hrule}}

% Statistics
\def\Prodint{\mathop{\mathchoice{\vcenter{\epsfysize=1.5em\epsfbox{%
  prodint.eps}}}{\vcenter{\epsfysize=1em\epsfbox{prodint.eps}}}{}{}}}
\def\prodint{\Prodint}
\def\tdot#1{\kern1.2pt\dot{\vphantom{#1}}\kern-1.2pt
        \dot#1\kern0.8pt\dot{\vphantom{#1}}\kern-0.8pt}
\def\contiguous{\triangleleft}
\def\doublecontiguous{\mathrel{\triangleleft\,\joinrel\triangleright}}
\def\E{\mathord{\rm E}}
\def\Pr{\mathord{\rm P}}
\def\var{\mathop{\rm var}\nolimits}
\def\sdev{\mathop{\rm sd}\nolimits}
\def\cov{\mathop{\rm cov}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\cor{\mathop{\rm cor}\nolimits}
\def\Cor{\mathop{\rm Cor}\nolimits}
\let\covar\cov
\let\Covar\Cov
\let\Var=\var
\def\med{\mathop{\rm med}\nolimits}
\def\medlimits{\mathop{\rm med}\limits}
\def\almostsurely{{\rm a.s.}}
\def\almosteverywhere{{\rm a.e.}}
\def\infinitelyoften{{\rm i.o.}}
\def\ae{\almosteverywhere}
\def\ldot{\hbox {$\dot \ell$}}
\def\ltil{\hbox{$\tilde \ell$}}
\def\dirac{\delta}
\def\haslaw{\sim}
\def\haslawunder#1{\mathchoice{\buildrel #1\over \sim}{\ \mathrel{^{#1}}\joinrel\sim}{}{}}
\def\generatedby{\s}
\mathchardef\given="626A
\mathcode`:="603A
%\mathchardef\setminus="2200


% Convergence symbols
\def\generalweak#1{\ {\mathchoice{\buildrel #1\over \rightsquigarrow}%
{\raise-2pt\hbox{$\buildrel #1\over \rightsquigarrow$}}{}{}}\ }
\let\weak\rightsquigarrow
\def\generalprob#1{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel#1\over\ra$}}
{\raise-2pt\hbox{$\buildrel#1\over\ra$}}{}{}}\ }
\def\outerp{\generalprob {\small P*}}
\def\prob{\generalprob{\small P}}
\def\outeras{\generalprob{\small as*}}
\def\as{\generalprob{\small as}}
\def\vague{\generalprob{\small v}}
\def\au{\generalprob{\small au}}
\def\Pgg{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel {\small P}\over\gg$}}
{\raise-2pt\hbox{$\buildrel {\small P}\over\gg$}}{}{}}\ }

% Miscellaneous
\def\beginskip{\begingroup\long\def\eet##1\endskip{\endgroup}\eet}
\def\endskip{}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1pt\vbox{\kern1pt #1\kern1pt}\kern1pt\vrule}\hrule}}
\def\eet#1{}
\def\makenumbersactive{\catcode`\0=11\catcode`\1=11\catcode`\2=11%
        \catcode`\3=11\catcode`\4=11\catcode`\5=11%
        \catcode`\6=11\catcode`\7=11\catcode`\8=11\catcode`\9=11 }



\catcode`\@=12








==> oldstuff/Consistency.tex <==
\section{Posterior consistency}\label{sec:consistency}
In order to apply our theorems we first need to show consistency of the posterior distribution. 
We provide two tools for that.
The first tool is based on combining two seminal results. 
The first result on which our work is based is Schwartz theorem~\cite{schwartzBayesProcedures1965} (see also the proof of~\cite[Lemma 6.16, 6.17]{ghosalFundamentalsNonparametricBayesian2017}).
This theorem is the standard result for showing that the posterior distribution is consistent.
The second result on which our work is based is the consistency theorem by Kiefer and Wolfowitz~\cite{kieferConsistencyMaximumLikelihood1956}.
This shows that the supremum of the likelihood ratio outside some small ball is exponentially small.
We will follow the discussion for the assumptions in the style of Kiefer-Wolfowitz. 
In the case of semiparametric mixtures, the $\gamma = (\theta, F)$.


\begin{assumption}\label{assumption_compactness}
  $\Gamma$ is a pre-compact metric space with metric $d$.
\end{assumption}

\begin{assumption}\label{assumption_density}
  For all $\gamma \in \Gamma$, $p_\gamma$ is a density with respect to a $\sigma$-finite measure $\mu$.  
\end{assumption}

\begin{assumption}\label{assumption_continuity}
  The map $\gamma \mapsto p_\gamma(x)$ is continuous for all $x$ and can be continuously extended to the compactification of $\Gamma$.
\end{assumption}

\begin{assumption}\label{assumption_identifiable}
  For all $\gamma_0, \gamma_1$ there exists $y$ such that 
  \[
    \int_{-\infty}^y p_{\gamma_1}(x) \dd \mu 
    \neq 
    \int_{-\infty}^y p_{\gamma_0}(x) \dd \mu 
  \]
\end{assumption}

\begin{assumption}\label{assumption_measurable_sup}
  The function
  \[
    w_{\gamma, \rho}(x) = \sup_{\gamma'|  d(\gamma, \gamma') < \rho } p_{\gamma'}(x)
  \]
  is measurable.
\end{assumption}

If $\gamma_0 \in \Gamma$ we denote the distribution with density $p_\gamma$ by $P_0 := P_{\gamma_0}$.

\begin{assumption}\label{assumption_integrability}
  For any $\gamma \in \Gamma$, we have
  \[
    \lim_{\rho \downarrow 0}
    \EE_{\gamma_0}\left[
      \log
      \frac{
        w_{\gamma, \rho}
      }{
        p_{\gamma_0}
      }(X)
    \right]
    < \infty
  \]
\end{assumption}


\begin{remark}\label{remark_LR_bound}
  Kiefer and Wolfowitz show in~\cite{kieferConsistencyMaximumLikelihood1956} that under~\Cref{assumption_compactness,assumption_density,assumption_continuity,assumption_identifiable,assumption_measurable_sup,assumption_integrability} there exists $h(\rho)$ such that $0< h(\rho) < 1$ such that eventually $[P_{\gamma_0}^\infty]$-almost surely
  \[
    \sup_{ \gamma | d(\gamma, \gamma_0)> \rho } \prod_{i = 1}^n \frac{p_\gamma}{p_{\gamma_0}} (X_i) < h(\rho)^n
  \]
\end{remark}

\begin{remark}\label{remark_Unormalized_posterior_mass}
  Following the proof of Schwartz theorem \cite[theorem 6.17]{ghosalFundamentalsNonparametricBayesian2017} we can prove that for any $\gamma_0$ that belongs to the Kullback-Leibler support of $\Pi$, for all $c' > 0$, eventually $[P_{\gamma_0}^\infty]$ a.s.:
  \[
    \int \prod_{i = 1}^n \frac{p_\gamma}{p_{\gamma_0}}(X_i) \dd \Pi(\gamma) \gtrsim e^{-c'n}
  \]
\end{remark}

\begin{remark}\label{remark:ConsistencyPerturbedPosterior}
    We can replace the almost sure argument from \cite[theorem 6.17]{ghosalFundamentalsNonparametricBayesian2017} by theorem 6.26 from the same reference. 
    This can be used to prove consistency for the perturbed models if this would be needed.
\end{remark}



\begin{proof}
  We begin the proof as in \cite[Theorem 6.17]{ghosalFundamentalsNonparametricBayesian2017}.
  Let $c'> 0$. Pick $0 < c < c'$ and set define $U = \{ p : \textrm{KL}(p_0; p) < c \}$. 
  Since $p_0$ belongs to the Kullback-Leibler support, it follows that $\Pi(U) > 0$. 
  Then we can write
  \[
    \int \prod_{i = 1}^n \frac{p}{p_0} (X_i) \dd \Pi(p) \geq \Pi(U) \int \prod_{i = 1}^n \frac{p}{p_0} (X_i) \dd \Pi_0(p),
  \]
  where $\Pi_0$ is the normalized restriction of $\Pi$ to $U$. 
  By Jensen's inequality its logarithm is bounded below by $\log \Pi(U) + \int \log \prod_{i = 1}^n \frac{p}{p_0}(X_i) \dd \Pi_0(p)$. 
  The second term times $n^{-1}$ coincides with the average $\frac{1}{n} \sum_{i = 1}^n \int \log \frac{p}{p_0}(X_i) \dd \Pi_0(p)$. 
  By Fubini's theorem the expectation is $- \int KL(p_0; p) \dd \Pi_0(p) \geq -c$. 
  Thus eventually almost surely, $\frac{1}{n} \sum_{i = 1}^n \int \log \frac{p}{p_0}(X_i) \dd \Pi_0(p) \geq - c'$.
  Therefore eventually almost surely
  \[
    \int \prod_{i = 1}^n \frac{p_\gamma}{p_{\gamma_0}}(X_i) \dd \Pi(\gamma) \gtrsim e^{-c'n}.
  \]

\end{proof}

\begin{lem}\label{lem:posteriorconsistency}
  Suppose that $\gamma_0$ belongs to the Kullback-Leibler support of $\Pi$ and that \Cref{assumption_compactness,assumption_density,assumption_continuity,assumption_identifiable,assumption_measurable_sup,assumption_integrability} are satisfied. Then the posterior distribution is consistent at $\gamma_0$.
\end{lem}

\begin{proof}
Let $\mathcal{U}$ be any open neighbourhood of $\gamma_0$. 
Using \cref{remark_LR_bound} and that there exists a $\rho$ such that the ball of radius $\rho$ centered at $\gamma_0$ is contained in $\mathcal{U}$, they show that there exists an $h = h(\rho)$ such that $0 < h< 1$ and eventually $[P_{\gamma_0}^\infty]$-almost surely:
  \begin{equation}
    \sup_{\gamma \in \mathcal{U}^c} \prod_{i = 1}^n \frac{p_{\gamma}}{p_{\gamma_0}}(X_i) < h^n. \label{step_LR_bound}
  \end{equation}
  Furthermore, by \Cref{remark_Unormalized_posterior_mass} there exists $0< c < -\log(h)$ such that eventually a.s. $[P_{\gamma_0}^\infty]$:
  \begin{equation}
    \int \prod_{i = 1}^n  \frac{p_\gamma}{p_{\gamma_0}}(X_i) \dd \Pi(\gamma) \gtrsim e^{-cn}. \label{step_unormalized_posterior_mass_bound}
  \end{equation}
 Then $[P_{\gamma_0}^\infty]$ almost surely:
  \begin{align*}
    \lim_{n \rightarrow \infty}
      \Pi(\mathcal{U}^c | X^n)
    &= 
    \lim_{n \rightarrow \infty}
      \frac{
        \int_{\mathcal{U}^c} \prod_{i = 1}^n \frac{p_\gamma}{p_{\gamma_0}}(X_i) \dd \Pi(\gamma)
      }{
        \int                 \prod_{i = 1}^n \frac{p_\gamma}{p_{\gamma_0}}(X_i) \dd \Pi(\gamma)
      }\\
      \intertext{Now we use \Cref{step_LR_bound,step_unormalized_posterior_mass_bound} and that $\log(h) + c < 0$}
    &\lesssim
     \lim_{n \rightarrow \infty}
     e^{(\log(h) + c) n} = 0
  \end{align*}
\end{proof}


\begin{lem}
  The posterior distribution $\Pi_n\left( \cdot \middle| X_1,\dots, X_n \right)$ in the model $X_1, \dots, X_n | p_\theta \sim p_\theta$ and $p\sim \Pi$ is strongly consistent at $p_{\theta_0}$ if all of the following hold:
  \begin{itemize}
    \item for any open $U$, $\sup_{\theta \in U^c} \text{KL}\left( p_{\theta} | p_{\theta_0} \right) > 0$;
    \item $\{\ell(\theta) | \theta \in \Theta \}$ is Glivenko-Cantelli;
    \item $\theta_0$ belongs to the Kullback-Leibler support of $\Pi$.
  \end{itemize}
\end{lem}

\begin{proof}
  Let $U$ be any open neighbourhood of $\theta_0$. Denote $c = \sup_{\theta \in U^c} \text{KL}\left( p_{\theta} | p_{\theta_0} \right) > 0$. Then for any $0< c' <c$, eventually almost surely $\sup_{\theta \in U^c} \left(\ell_n(\theta) - \ell_n(\theta_0)\right) \leq c'$, and therefore $\int_{U^c} \prod_{i = 1}^n \frac{p_{\theta}}{p_{\theta_0}} (X_i) \dd \Pi(\theta) \leq \int_{U^c} e^{-c'n} \dd \Pi(\theta) \leq e^{-c'n}$. Now apply \Cref{remark_Unormalized_posterior_mass} and finish the proof as usual.
\end{proof}



==> oldstuff/DesiredTheorem.tex <==
\section{Desired Theorem}
Let $F\sim\DP(\a)$ and independently $\q\sim \Pi$, and suppose we have
observations $X_1,\ldots,X_n\given F,\q\iid p_{\q,F}$. For a given differentiable function $\chi$, we
wish to prove that, in $P_{\q_0,F_0}^n$-probability
\[\sqrt n\bigl(\chi(\q)-\chi(\q_0)-\PP_n\dot\chi_{\q_0}\tilde I_{\q_0,F_0} ^{-1}\tilde\ell_{\q_0,F_0} \bigr)\given X_1,\ldots,X_n
\weak N\bigl(0, \dot\chi_{\q_0} \tilde I_{\q_0,F_0}^{-1}\dot\chi_{\q_0}^T\bigr).\]
Here $\tilde\ell_{\q,F}$ is the efficient score function,
and $\tilde I_{\q,F}=P_{\q,F}\tilde\ell_{\q,F}\tilde\ell_{\q,F}^T$ is the efficient information.

Proof idea, following Castillo, written for the case that $\chi(\q)=\q$ and for one-dimensional $\q$. 
The Laplace transform of the posterior distribution on the left is
\begin{align*}
  I_n(\l)&= 
    \EE\bigl(
      e^{
        \l\sqrt{n}(\q-\q_0)
        -
        \l\ep_n \tilde{I}_{\q_0,F_0}^{-1}  \tilde\ell_{\q_0,F_0} 
      }
\given X_1,\ldots,X_n\bigr).
\end{align*}
It suffices to show that this tends to the Laplace transform $\exp(\thalf \l^2\tilde I_{\q_0,F_0}^{-1})$, 
of the normal distribution, for every $\l$ in a neighbourhood of 0. 

Let $t\mapsto F_t(F)$ so that 
(at least at $(\q_0,F_0)$?)
$$\frac{\partial}{\partial t}_{|t=0}\log p_{\q+t,F_t(F)}(x)=\tilde\ell_{\q,F}.$$
For $\ell_n(\q, F)=\log \prodin p_{\q,F}(X_i)$ the log likelihood, we rewrite the Laplace
transform at $\tilde I_0\l$ as, with $\tilde\ell_0=\tilde \ell_{\q_0,F_0}$ and $\tilde I_0=\tilde I_{\q_0,F_0}$
\begin{align*}
&\frac{\int\!\!\int e^{\tilde I_0\l\sqrt n (\q-\q_0)-\l\ep_n\tilde \ell_0 
+\ell_n(\q,F)-\ell_n(\q+n^{-1/2}\l,F_{n^{-1/2}\l}(F))}\,
e^{\ell_n(\q+n^{-1/2}\l,F_{n^{-1/2}\l}(F))}\,\Pi(\q)\,d\Pi(F)}
{\int\!\!\int e^{\ell_n(\q,F)}\,d\Pi(\q)\,d\Pi(F)}.
\end{align*}
This is a trivial rewrite, which is true for any submodel, but the point is that for the given
least favourable submodel we hope that it is true that
\begin{align*}
\ell_n(\q+n^{-1/2}\l ,F_{n^{-1/2}\l}(F))-\ell_n(\q,F)&=\tilde I_0\l \sqrt n (\q-\q_0)-\l \ep\tilde \ell_0 
-\thalf \l^2\tilde I_0+o_P(1),\\
\frac{\int\!\!\int e^{\ell_n(\q+n^{-1/2}\l,F_{n^{-1/2}\l}(F))}\,d\Pi(\q)\,d\Pi(F)}{\int\!\!\int e^{\ell_n(\q,F)}\,d\Pi(\q)\,d\Pi(F)}
&\prob 1.
\end{align*}
If these would be true, the first one uniformly in $(\q,F)$, then the desired result would follow, because
by the first we can replace the first exponential in the integral in the numerator by $e^{\thalf\l^2\tilde I_0}$, 
and next use the second to cancel the integrals in the numerator and denominator. As the first is a Taylor
expansion, it is definitely needed to show consistency of the posterior as a preliminary step.
If it can be shown that the posterior distribution concentrates on certain subsets of $(\q,F)$,
then the uniformity can be restricted to these sets. 

The second condition is the ``change of measure''
condition on the prior: it requires that the prior does not change much 
``in the direction of the least favourable direction''. For Gaussian process priors, this requires
careful consideration, using results on Gaussian concentration, and it would hold only if misspecification of the
prior does not introduce bias in the posterior of $\q$. What does it mean in the case of the Dirichlet?
Are the results in Ray et al of help?

We can rewrite the first requirement as
\begin{align*}
&\ep_n\Bigr[\sqrt n\bigl(\log p_{\q+n^{-1/2}\l ,F_{n^{-1/2}\l}(F)}-\log p_{\q,F}\bigr)-\l\tilde\ell_0\Bigr]\\
&\qquad+n P_0\bigl(\log p_{\q+n^{-1/2}\l ,F_{n^{-1/2}\l}(F)}-\log p_{\q,F}\bigr)-\tilde I_0\l \sqrt n (\q-\q_0)
-\thalf \l^2\tilde I_0=o_P(1).
\end{align*}
The random part should be something like $\l \tilde\ell_{\q,F}$ by the construction of $F_t(F)$, and
$\ep_n(\tilde\ell_{\q,F}-\tilde\ell_0)$ should tend to zero, if $(\q,F)\ra (\q_0,F_0)$. For uniformity
we would impose a Donsker type condition, or study the entropy of the class of functions involved 
(in its dependence on $n$).
The more tricky part may be the deterministic term in the second line.

A two-term Taylor expansion suggests
$$nP_0\bigl(\log p_{\q+n^{-1/2}\l ,F_{n^{-1/2}\l}(F)}-\log p_{\q,F}\bigr)
\approx \sqrt n\l P_0\tilde\ell_{\q,F}+\thalf \l^2P_0\frac{\partial}{\partial\q}\tilde\ell_{\q,F}.$$
Differentiating the identity $P_{\q,F}\tilde\ell_{\q,F}=0$ with respect to $\q$ gives
$$P_{\q,F}\frac{\partial}{\partial\q}\tilde\ell_{\q,F}=-P_{\q,F}\tilde\ell_{\q,F}\dot\ell_{\q,F}=-\tilde I_{\q,F}.$$
Thus the last term on the right should be asymptotic to $-\thalf\l^2\tilde I_0$.
The first term on the right is
\begin{align*}
\sqrt n\l P_0\tilde\ell_{\q,F}&=\sqrt n\l P_0(\tilde\ell_{\q,F}-\tilde\ell_{\q_0,F})+\sqrt n P_0\tilde\ell_{\q_0,F}\\
&\approx\sqrt n(\q-\q_0)\l P_0\frac{\partial}{\partial\q}\tilde\ell_{\q,F}{}_{|\q=\q_0}+\sqrt n P_0\tilde\ell_{\q_0,F}.
\end{align*}
Thus the desired result seems to follow provided $\sqrt n P_0\tilde\ell_{\q_0,F}$ tends to zero. This
is a version of the no-bias condition, which also popped up in the analysis of the maximum likelihood estimator.
In the mixture models we consider here, the condition is automatically satisfied. Indeed
$\tilde\ell_{\q,F}$ is orthogonal to all score functions for $F$, which include the scores $p_{\q,G}/p_{\q,F}-1$. Thus,
for every $F,G$,
$$P_{\q,G}\tilde\ell_{\q,F}
=\int \Bigl(\frac{p_{\q,G}}{p_{\q,F}}-1\Bigr)\tilde\ell_{\q,F}\,dP_{\q,F}=0.$$



==> oldstuff/ExponentialFrailty.tex <==
\section{Exponential Frailty}
We observe a sample from the distribution of $(X,Y)^T$, where given $Z$ the variables
$X$ and $Y$ are independent and exponentially distributed with intensities $Z$ and $\q Z$.
Hence $F$ is a distirbution on $(0,\infty)$ and $\q>0$.

In the mixture model case, the kernel is given by
\[
  p_{\theta}(x, y | z) = z e^{-zx} \theta z e^{- \theta z y} = z^2 \theta e^{-z(x + \theta y)}.
\]
This leads to a mixing distribution of the form
\[
  p_{\theta, F} (x,y) = \int  z^2 \theta e^{-z(x + \theta y)} \dd F(z).
\]
The least favourable submodel is known explicitly. See \cite{vandervaartEfficientMaximumLikelihood1996}. 


\subsection{Kullback-Leibler support}
In order to apply the results, we need to show that there is a big enough Kullback-Leibler support.
\begin{lem}\label{lem:frailty_finite_support_approx}
  For every $F$ on $[m,M]$ and $0 < \epsilon < \frac{1}{2}$ there exists a discrete $F_\epsilon$ with fewer than $C \frac{M}{m} \log \frac{1}{\epsilon}$ support points such that \[ \| p_F - P_{F_\epsilon} \|_1 < \epsilon. \]
\end{lem}

\begin{proof}
  Let $K > 0$ be an integer. Then 
  \[
    e^{-x} = \sum_{i = 1}^{K-1} \frac{x^i}{i!} + R_k(x),
  \]
  with $R(x) = e^{\xi_{K,x} x^K}{K!}$, where $0 < \xi_{K, x} < 1$.
  Suppose the first $K$ moments match: 
  \[
    \int z^2 z^i \dd F(z) = \int z^2 z^i \dd G(z), \quad i = 0, \dots, K-1.
  \]
  Then we can bound the $L_1$ distance between the $P_F$ and $P_G$:
  \[
    \|
    \int z^2 e^{-xz} \dd (F - g)(z)
    \|_1
    \leq
    \int \frac{|xz|^K}{K!} \dd (F + G)(z)
  \]
  If we pick $G$ to also be supported on $[m, M]$ we can bound this further by: 
  \[
    2 \frac{(x M)^K}{K!}. 
  \]

\end{proof}<++>


==> oldstuff/LikelihoodExpansion.tex <==
\subsection{Verifying \Cref{EqRemainders}}\label{sec:LAN}


Condition \eqref{EqRemainders} can be split in a random and a deterministic part: 
\begin{align}
&\ep_n\Bigr[\sqrt n\log \frac{p_{\q+n^{-1/2}t ,F_{n^{-1/2}t}(\q,F)}}{p_{\q,F}}-t^T\tilde\ell_0\Bigr]
=o_P(1),\label{EqRandomPart}\\
&n P_0\log \frac{p_{\q+n^{-1/2}t ,F_{n^{-1/2}t}(\q,F)}}{p_{\q,F}}=-t^T\bigl(\tilde I_0+o_P(1)\bigr) \sqrt n (\q-\q_0)
-\thalf t^T\tilde I_0t+o_P(1).\label{EqDeterministicPart}
\end{align}
The $o_P(1)$ terms should tend to zero in $P_{\q_0,F_0}^n$-probability, uniformly in $(\q,F)\in \Theta_n\times\F_n$.
The uniformity in \eqref{EqRandomPart} can be proved by showing that the relevant set of functions
are contained in a Donsker class, or through entropy conditions. The following lemma
gives sufficient conditions in terms of a Donsker class.

\begin{lem}\label{Lem:LANByDonsker}
Suppose that the map $t\mapsto \ell(t;\q,F)(x):=\log p_{\q+n^{-1/2}t ,F_{n^{-1/2}t}(\q,F)}(x)$ is twice continuously differentiable in
a neighbourhood of zero, for every $(\q,F)\in \Theta_n\times\F_n$ and $x\in\X$.
\begin{itemize}
\item If the classes of functions $\{\dot\ell(t/\sqrt n;\q,F): \|t\|<1, (\q,F)\in\Theta_n\times\F_n\}$ are
contained in a given $P_0$-Donsker class and $P_0\|\dot\ell(t_n/\sqrt n;\q_n,F_n)- \tilde\ell_0\|^2\ra 0$,
for every $\|t_n\|<1$ and $(\q_n,F_n)\in\Theta_n\times\F_n$, then 
\eqref{EqRandomPart} is valid. 
\item If $\|P_0\ddot\ell(t_n/\sqrt n;\q_n,F_n)- \tilde  I_0\|\ra 0$, 
for every $\|t_n\|\le 1$ and $(\q_n,F_n)\in\Theta_n\times\F_n$, then \eqref{EqDeterministicPart} is satisfied if also
$$\sup_{\q\in\Theta_n,F\in\F_n} \frac{\|P_0\dot\ell(0;\q,F)+\tilde I_0(\q-\q_0)\|}
{\|\q-\q_0\|+n^{-1/2}}\stackrel {P_0^n}\longrightarrow 0.$$
\end{itemize}
%$\{\ddot\ell(t/\sqrt n;\q,F): \|t\|<1, (\q,F)\in\Theta_n\times\F_n\}$ are contained in a $P_0$-Glivenko-Cantelli class
\end{lem}


\begin{proof}
The left side of \eqref{EqRandomPart} is equal to 
$$\sqrt n\ep_n\Bigl[\ell\Bigl(\frac t{\sqrt n};\q,F\Bigr)-\ell(0;\q,F)\Bigr]-t^T\ep_n\tilde\ell_0
=t^T\ep_n\int_0^1 \Bigl[\dot\ell\Bigl(\frac{st}{\sqrt n}; \q,F\Bigr)-\tilde\ell_0\Bigr]\,ds.$$ 
If the classes of functions $\{\dot\ell(t/\sqrt n;\q,F): \|t\|<1, (\q,F)\in\Theta_n\times\F_n\}$ are contained in
a fixed Donsker class, then the convex hull relative to $t$ of these classes are contained in the
convex hull of the latter Donsker class, which is also Donsker. Thus the 
classes of functions $\int_0^1 (\dot\ell(st/\sqrt n; \q,F)-\tilde\ell_0)\,ds$ are contained in
a Donsker class. Their empirical process tends to zero, as 
$\sup_{|t\|<1}P_0\|\dot\ell(t/\sqrt n;\q_n,F_n)- \tilde\ell_0\|^2\ra 0$, by assumption.

By a second-order Taylor expansion we can write the left side of \eqref{EqDeterministicPart} as
$$nP_0\Bigl[\ell\Bigl(\frac t{\sqrt n};\q,F\Bigr)-\ell(0;\q,F)\Bigr]=\sqrt n\, t^TP_0\dot\ell(0;\q,F)
+t^T\!\int_0^1 P_0\ddot\ell\Bigl(\frac{st}{\sqrt n}; \q,F\Bigr)(1-s)\,ds\, t.$$
The first term on the right is $-t^T\bigl(\tilde I_0+o_P(1)\bigr)\sqrt n(\q-\q_0)+o_P(1)$, by assumption.
The second term is $t^T\tilde I_0 t/2+o_P(1)$, by the assumption that
$\sup_{\|t\|\le 1}\|P_0\ddot\ell(t/\sqrt n;\q_n,F_n)- \tilde  I_0\|\ra 0$.
\end{proof}

For an exact least favourable submodel $t\mapsto F_t(\q,F)$, the derivative $\dot\ell(0;\q,F)$ is equal
to the efficient score function $\tilde \ell_{\q,F}$. Then the displayed condition in the lemma is satisfied if
$\Theta_n$ shrinks to $\q_0$ and, as uniformly in $F\in\F_n$, as $\q\ra\q_0$,
$$P_{\q_0,F_0}\tilde\ell_{\q,F}=-\tilde I_0 (\q-\q_0)+o_P\bigl(\|\q-\q_0\|+n^{-1/2}\bigr).$$
There are two ways in which we can verify this, both starting from the fact that
$P_{\q,F}\tilde\ell_{\q,F}=0$, for every $(\q,F)$. The first is to write the left side as
$$P_{\q_0,F_0}(\tilde\ell_{\q,F}-\tilde\ell_{\q_0,F})+P_{\q_0,F_0}\tilde\ell_{\q_0,F}
\approx P_{\q_0,F_0}\dot{\tilde\ell}_{\q_0,F_0}(\q-\q_0)+P_{\q_0,F_0}\tilde\ell_{\q_0,F}.$$
Here $P_{\q_0,F_0}\dot{\tilde\ell}_{\q_0,F_0}=-\tilde I_0$, as follows from differentiating 
across the identity $P_{\q,F}\tilde\ell_{\q,F}=0$, and the fact that $P_{\q,F}\tilde\ell_{q,F}\dot\ell_{\q,F}^T=\tilde I_{\q,F}$,
for $\dot\ell_{\q,F}$ the ordinary score function for $\q$.
The second way is to write the left side as
$$(P_{\q_0,F_0}-P_{\q,F_0})\tilde\ell_{\q,F}+P_{\q,F_0}\tilde\ell_{\q,F}
\approx -P_{\q_0,F_0}\tilde\ell_{\q_0,F_0}\dot\ell_{\q_0,F_0}^T(\q-\q_0)+P_{\q,F_0}\tilde\ell_{\q,F}.$$
In both ways the term on the far right will be required to be $o(n^{-1/2})$, which is a 
a version of the ``no-bias condition'', which also popped up in the analysis of the maximum likelihood estimator.
This may require a rate of convergence of $F\in\F_n$ to $F_0$ (typically $o(n^{-1/4}$, because the first derivative
with respect to $F$ should vanish in view of the orthogonality of $\tilde \ell_{\q,F}$ to score functions
for $F$), but structural properties of the model determine may help. 
In the mixture models we consider here, the term is actually identically zero. Indeed
$\tilde\ell_{\q,F}$ is orthogonal to all score functions for $F$, which include the scores $p_{\q,G}/p_{\q,F}-1$. Thus,
for every $F,G$,
$$P_{\q,G}\tilde\ell_{\q,F}
=\int \Bigl(\frac{p_{\q,G}}{p_{\q,F}}-1\Bigr)\tilde\ell_{\q,F}\,dP_{\q,F}=0.$$

Next, we will provide a lemma that is useful for the computations. To apply \Cref{Lem:LANByDonsker} we need to compute the gradient and the hessian matrix. The following lemma provides a strategy for computing these. 

\begin{lem}\label{lem:ExpressionsForGradiantHessian}
    Suppose that $p_{\theta}(x \given z) = e^{h_\theta(x \given z)}$, and that the perturbation in the least favourable submodel is given by $p_{\theta + t, F_t}(x) = \int p_{\theta + t} (x \given \phi_{t,\theta}(z)) \dd F(z)$. Denote $D_{t, \theta} (x \given z) := \nabla_t h_{\theta + t}( x \given \phi_{t, \theta}(z))$. Then, whenever the functions within the integrals are dominated by an $F(z)$ integrable function:
    \[
        \nabla_t p_{\theta + t, F_t}(x) = \frac{\int e^{h_{\theta+t}(x \given \phi_{t,\theta}(z))} D_{t, \theta} (x \given z) \dd F(z)}
        {
            p_{\theta + t, F_t}(x)
        }.
    \]
    and
    \begin{align*}
        H_t p_{\theta + t, F_t}(x) &= 
          \frac{ 
              \int e^{h_{\theta + t}(x \given \phi_{t, \theta}(z))} \left(H_t(h_{\theta + t}(x \given \phi_{t, \theta}(z)) + D_{t, \theta}(x \given z) D_{t, \theta}^T(x\given z) \right) \dd F(z)
              }{
              p_{\theta + t, F_t}(x)
          }\\
          &+ \left(\nabla_t p_{\theta + t, F_t}(x)\right) \left( \nabla_t p_{\theta + t, F_t}(x) \right)^T
    \end{align*}
\end{lem}

\begin{proof}
   Use the chain rule to compute the gradient and the Hessian of $\log(f)$. 
   This gives $\frac{f'}{f}$ and $\frac{ f''}{f} - \left( \frac{f'}{f} \right) \left( \frac{f'}{f} \right)^T$. 
   Set $f(t) = \int e^{h(t,z)} \dd F(z)$, so that 
   \begin{align*}
       f' &= \nabla_t \int e^{h(t,z)} \dd F(z),\\
       f'' &= H_t \int e^{h(t,z)} \dd F(z) = \nabla_t^T f'.
   \end{align*}
   Next we use the dominated integrability to apply the Leibniz rule and move the differentiating inside the integration sign and apply the chain rule. This gives
   \begin{align*}
       f' &= \int e^{h(t,z)} \nabla_t h(t,z) \dd F(z), \\
       f'' &= \int e^{h(t,z)} \left( \nabla_t^T \nabla_t h(t,z) + \left(\nabla_t h(t,z)\right) \left(\nabla_t h(t,z)\right)^T \right) \dd F(z).
   \end{align*}
   Filling in the definitions in as in the assumptions gives the final result.
\end{proof}

To study the asymptotic behaviour of the derivatives of the log likelihood in $P_{\theta_0, F_0}$, we can use the following lemma:
\begin{lem}\label{lem:LimitsOfExpectationsLogLik}
    Let $p_{\theta}(x \given z) = e^{h_\theta(x \given z)}$ be the mixture kernel, and the perturbation in the least favourable submodel given by $p_{\theta + t, F_t} = \int p_{\theta + t}(x \given \phi_{t, \theta}(z)) \dd F(z)$.
    Suppose that $h_{\theta}(x \given z)$ is twice continuously differentiable in $(\theta, z)$,
    and that $\phi_{t,\theta}(z)$ is twice continuously differentiable in $t, \theta$.
    Furthermore, assume that the maps $z \mapsto \nabla_t p_{\theta + t}(x \given \phi_{t, \theta}(z)) \given_{t = t_n/\sqrt{n}}$ and $z \mapsto H_t p_{\theta + t}(x \given \phi_{t, \theta}(z))\given_{t = t_n/\sqrt{n}}$ are bounded for all $x$, $| t_n| \leq 1$ and $\theta \in \Theta_n$.
    Finally, assume that $\nabla_t \log p_{\theta + t, F_t}(x) \given_{t = t_n/\sqrt{n}}$ and $H_t \log p_{\theta + t, F_t}(x) \given_{t = t_n/\sqrt{n}}$ have envelope functions that are square integrable and integrable respectively.
    Then for all $|t_n| \leq 1$, $\theta_n \rightarrow \theta_0, F_n \rightsquigarrow F_0$:
    \begin{align*}
        P_{\theta_0, F_0} \| \dot\ell( t_n/\sqrt{n} ; \theta_n, F_n) - \ell_0 \|^2 &\rightarrow 0 \\
        \|P_{\theta_0, F_0} \ddot\ell(t_n/\sqrt{n} ; \theta_n, F_n) - \tilde{I}_0 \|&\rightarrow 0.
    \end{align*}
\end{lem}

\begin{proof}
    We use the explicit expressions found in \Cref{lem:ExpressionsForGradiantHessian}.
    By the chain rule, continuity, integrability and weak convergence we can conclude that pointwise
    \begin{align*}
        \dot\ell( t_n/\sqrt{n} ; \theta_n, F_n)(x) - \dot\ell (0; \theta_0, F_0)(x) &\rightarrow 0 \\
        \ddot\ell(t_n/\sqrt{n} ; \theta_n, F_n)(x) - \ddot\ell(0; \theta_0, F_0)(x) &\rightarrow 0.
    \end{align*}
    Next, we use the pointwise limits, the envelope functions together with the dominated convergence theorem
    \begin{align*}
        P_{\theta_0, F_0} \| \dot\ell( t_n/\sqrt{n} ; \theta_n, F_n) - \dot\ell(0; \theta_0, F_0) \| &\rightarrow 0\\
        P_{\theta_0, F_0} \| \ddot\ell(t_n/\sqrt{n} ; \theta_n, F_n) - \ddot\ell(0;\theta_0, F_0) \| &\rightarrow 0
    \end{align*}
    By using that $\ell_0 = \dot\ell(0; \theta_0, F_0)$ and $P_{\theta_0, F_0} \ddot\ell(0; \theta_0, F_0) = \tilde{I}_0$, we finally get the results as claimed:
    \begin{align*}
        P_{\theta_0, F_0} \| \dot\ell( t_n/\sqrt{n} ; \theta_n, F_n) - \ell_0 \|^2 &\rightarrow 0 \\
        \|P_{\theta_0, F_0}  \ddot\ell(t_n/\sqrt{n} ; \theta_n, F_n) - \tilde{I}_0 \|&\rightarrow 0.
    \end{align*}

\end{proof}


==> oldstuff/Mixtures.tex <==

\section{Mixtures}
Suppose we observe a random sample from a mixture density of the form
\begin{equation}
  x\mapsto p_{\q,F}(x):=\int p_\q(x\given z)\, dF(z).\label{eq:mixingdensity}
\end{equation}
The kernel $x\mapsto p_\q(x\given z)$ is the (known) density of a random variable $X$ given 
a latent random variable $Z$, which has marginal distribution $F$. 
The kernel is indexed by a parameter  $\q\in\RR^d$ that we  wish to  estimate.


One possible estimator is the full maximum likelihood estimator, which 
given a sample $X_1,\ldots, X_n$ from the distribution of $X$, maximizes the likelihood
\[
  (\q,F)\mapsto \prodin \int p_\q(X_i\given z)\,dF(z). 
\]
These estimators were shown to be consistent in some generality in~\cite{kieferConsistencyMaximumLikelihood1956}.
For a small number of special models the $\q$-component of the maximum likelihood
estimator is known to be asymptotically normal and efficient from~\cite{vandervaartEstimatingRealParameter1988,murphyLikelihoodInferenceErrorsinVariables1996,vandervaartEfficientMaximumLikelihood1996}. 

A Bayesian alternative is to equip $F$ with a species sampling prior, and, independetly $\theta$ with a smooth prior.
Two common choices for a mixture prior would be the Dirichlet process prior or a finite discrete prior with a random number of components.
These two choices are the priors we will study in our examples.

The Dirichlet process is a stochastic process characterised by two parameters, the prior precision $M$ and the center measure $G$.
Then a random variable $F$ is said to be Dirichlet process distributed if for any partition $A_1, \dots A_k$
\[
    (F(A_1),\dots, F(A_k)) \sim \textrm{Dir}\left(k; MG(A_1),\dots, MG(A_k)\right).
\]

As an example of a finitely discrete prior with a random number of components, pick $\lambda, \sigma > 0$ and $G$ a probability distribution.
Then we draw $K \sim \textrm{Geom}(\lambda)$, and given $K$ draw $Z_1, \dots, Z_K \overset{\textrm{i.i.d.}}\sim G$, $W \sim \textrm{Dir}(K; \sigma,\dots, \sigma)$.
Then 
\[
    F = \sum_{i = 1}^K W_i \delta_{Z_i}
\]

More generally, a species sampling process can be defined using the exchangeable partition probability function (EPPF) and a center measure $G$.
There are many more examples of species sampling process priors, for example the Pitman-Yor processes, Gibbs processes or Poisson-Kingman processes.
For more details, see \cite[Chapter 14]{ghosalFundamentalsNonparametricBayesian2017}.

To show the asymptotical optimality of the Bayesian methodology, we prove a Bernstein-von Mises theorem for $\theta$.
Roughly, a Bernstein-Von mises theorem describes the asymptotic shape of the posterior.
For our purposes, we will show that, after rescaling by a $\sqrt{n}$ blow-up, the posterior will be a Gaussian centred on an efficient estimator with the inverse efficient fisher information as variance.


There are many examples of this structure. In some cases the information structure
is well travelled, and one would hope to get a result by following the proof by Castillo et al. (developed for
smooth priors)  and possibly Ray et al (developed for the Dirichlet, but with observed $Z$, so different?). 
In other cases it may be more difficult. We give some examples.

These approaches are based on perturbations of the least favourable submodel for $\q$.
The score for $\q$ is defined, as usual, as
\[\dot\ell_{\q,F}(x)=\frac{\partial}{\partial \q}\log p_{\q,F}(x)
=\frac{\int \dot\ell_\q(x\given z)\,p_\q(x\given z)\,dF(z)}{\int p_\q(x\given z)\, dF(z)}.
\]
Similarly score functions for $F$ are derivatives along submodels that perturb $F$. 

The efficient score function $\tilde\ell_{\q,F}$ for $\q$ is defined as the ordinary score minus its
projection onto the closed linear span of all score functions for $F$.
A least favourable submodel at $(\q, F)$ is a submodel given by parameters
$t\mapsto (\q+t, F_t)$, with $F_0=F$, such that 
\[
  \tilde\ell_{\q,F}(x)=\frac{\partial}{\partial t}_{|t=0}\log p_{\q+t,F_t}(x).
\]
It would be nice to know this explicitly, as conditions for the Bernstein-von Mises theorem 
have been stated in terms of a least favourable submodel.
In some examples we are interested in estimating only part of a vector-valued
parameter $\q$, and we are interested in a least favourable submodel for this part.

The one-dimensional submodel defined  by $dF_t(1+t b)\,dF$, for a given bounded function $b$ with $\int b\,dF=0$
and $t$ in a neighbourhood of zero, gives as score at $t=0$
\[
  A_{\q,F}b(x):=\frac{\partial}{\partial t}_{|t=0}\log p_{\q,F_t}(x)
=\frac{\int p_\q(x\given z)\,b(z)\,dF(z)}{\int p_\q(x\given z)\, dF(z)}.
\]
By varying $b$ we obtain a large class of score functions. By using perturbations of the
form $dF_t=c_t\chi(tb)\, dF$ for a given nonnegative function 
$\chi$ with $\chi(0)=\chi'(0)=1$, the requirement that $b$ be bounded can be dropped.
So any function as in the display with $\int b\,dF=0$ is a score function for $F$.

These perturbations preserve the support of $F$ and do not exhaust the possibilities.
One-sided submodels can be obtained using $F_t=(1-t)F+tG$, for $t\in [0,1]$, and deliver score
functions 
\[\frac{\partial}{\partial t}_{|t=0}\log p_{\q,F_t}(x)=\frac{p_{\q,G}}{p_{\q,F}}(x)-1
=\frac{\int p_\q(x\given z)\,dG(z)}{\int p_\q(x\given z)\, dF(z)}-1.\]
The limit must be taken for $t\da 0$, and so one cannot obtain the negative of this function
by inserting $-t$ instead of $t$, in general. For the efficient score function this is not important,
as this is defined through projection onto the linear space of all score functions. 
(The space of all these score functions is convex, which is enough for local asymptotic minimax theory.)
However, for the existence of a least favourable submodel and a Bernstein-von Mises proof, it may be.

We may similarly consider location or scale changes of $F$ (both two-sided), or yet other perturbations.




==> oldstuff/Neymann-Scott.tex <==
\section{Neyman-Scott}
Suppose the distribution of $X$ given $Z$ is bivariate normal with mean vector $(Z,Z)^T$ and
covariance matrix $\q^2 I$. The model is infamous because the direct maximum likelihood estimator
of $\q$ when  treating the  $n$ latent variables as unknown parameters, is inconsistent.

A simple efficient estimator is obtained by removing the latent variable by differencing:
$X_1-X_2$ possesses a $N(0,2\q^2)$-distribution, and the maximum likelihood estimator 
 $\thalf n^{-1}\sumin (X_{1i}-X_{2i})^2$ of $\q^2$ based on a sample of differences, is asymptotically efficient.
It is a little academic to consider a Bayesian approach using a Dirichlet prior on $F$.
The main question would be if the good properties of the simple estimator will not be
destroyed by a fancy Bayesian approach. However, the question does have intellectual appeal,
and the model may be a good test case.

We can transform from the original observation $X=(X_1, X_2)^T$ to the pair
$(X_1-X_2, X_1+X_2)$, which given $Z$ has a bivariate normal distribution with mean vector $(0, 2Z)$
and covariance matrix $2\q^2 I$. For simplicity of notation, drop the factors $2$ and denote
the transformed observation by $(X,Y)^T$.

Thus assume that $(X,Y)^T$ given $Z$ possesses a bivariate normal distribution with mean vector $(0,Z)$
and covariance matrix $\q^2 I$. The score function for $\q$ is given by 
\begin{align*}
\dot\ell_{\q,F}(x,y)&=\frac{\partial}{\partial \q}\log p_{\q,F}(x,y)\\
&=-\frac 1{\q}+\frac{x^2}{\q^3}
+\frac{\int\bigl (-1/\q+(y-z)^2/\q^3\bigr)\,\phi\bigl((y-z)/\q\bigr)\,dF(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)}\\
&=-\frac 2{\q}+\frac{x^2+y^2}{\q^3}
-\frac{2y}{\q^3}\frac{\int z\phi\bigl((y-z)/\q\bigr)\,dF(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)}
+\frac 1{\q^3}\frac{\int z^2\phi\bigl((y-z)/\q\bigr)\,dF(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)}.
\end{align*}
Scores functions for $F$ are functions of $y$ only, and include all functions of the types
\begin{align*}
\frac{\int \phi\bigl((y-z)/\q\bigr)\,b(z)\, dF(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)},\\
\frac{\int \phi\bigl((y-z)/\q\bigr)\, dG(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)}-1.
\end{align*}
The closed linear span of all these functions is the space of all mean zero functions of $y$.
This follows, because if $g$ is perpendicular in $L_2(p_{\q,F})$ to all functions of the second type and has
$\int g(y)\,p_{\q,F}(y)\,dy=0$, then,
$$0=\int g(y)\Bigl(\frac{p_{\q, G}(y)}{p_{\q,F}(y)}-1\Bigr)\,p_{\q,F}(y)\,dy=\int\!\!\int g(y)\, \phi\bigl((y-z)/\q\bigr)/\q\, dG(z)\,dy.$$
Hence $\int g(y)\, \phi\bigl((y-z)/\q\bigr)/\q\,dy=0$, for every $z$. 
The completeness of the normal location family then shows that $g=0$ almost everywhere.

It follows that the efficient score function for $\q$ is given by
$$\tilde\ell_{\q,F}(x,y)=-\frac 1{\q}+\frac{x^2}{\q^3}.$$
Does a least favourable submodel exist?

Perturbing the  location of $F$ gives the $F$-score
$$\frac{\int \phi'\bigl((y-z)/\q\bigr)/\q^2\,dF(z)}{\int \phi\bigl((y-z)/\q\bigr)/\q\, dF(z)}
=-\frac y{\q^2}+\frac{1}{\q^2}\frac{\int z\phi\bigl((y-z)/\q\bigr)\,dF(z)}{\int \phi\bigl((y-z)/\q\bigr)\, dF(z)}.$$
But is $y^2$ also a score (after centering) ?





==> oldstuff/SemiparametricBvMDP.tex <==


\subsection{Verifying \cref{EqChangeOfMeasure} for Species sampling processes}\label{sec:changeofmeasure}
The following lemma allows us to verify the BvM if $F_t$ is a coordinate transform of $F$, it is consistent under the coordinate changes and it does not create too many clusters in the posterior.
We will formalise these assumptions as to be able to discuss them.

\begin{assumption}\label{ass:ChangeOfVariables}
If $F_t$ is the map as in \Cref{EqChangeOfMeasure}, we assume that $ p_{\theta +t, F_t}(X) = \int p_{\theta + t}(x \given \phi_{t, \theta}(z)) \dd F(z)$ \end{assumption}
Under this assumption $\phi_{t,\theta}$ defines a change of variables of the latent variables.
This is equivalent to applying this change of variables to the center measure $G$ of the species sampling process. 
Denote the prior that we get after changing the coordinates by $\Pi_{t, \theta}$.

\begin{assumption}\label{ass:Smoothness}
    For $h$ the density of the prior $\pi$ and $G$ the center measure of the species sampling process with density $g$, we assume that there exists a open set $U$ of $\theta$ and constants $C_t, C'_t > 0$ such that, for all $\theta \in U$ and all $z$
     \begin{align}
         \left\| \frac{g( \phi^{-1}_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \left\| \det \dot \phi^{-1}_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z) \right\|}{g(z)} - 1  \right\| &\leq \frac{C_t}{\sqrt{n}};\label{ass:smoothnessinG}\\
        \left\| \frac{h( \theta + \frac{t}{\sqrt{n}})}{h(\theta)} - 1 \right\| & \leq \frac{C'_T}{\sqrt{n}}.\label{ass:smoothnessinh}
    \end{align}
\end{assumption}
The first condition is needed for a compatibility of the change of coordinates with the center measure.
This is needed to ensure that the errors will vanish.
The second condition is fairly weak, it is implied by a local log lipschitz condition on the prior density. See \Cref{lem:SmoothnessInG,lem:SmoothnessInH} for tools for verifying these assumptions.

For our argument to work, we need to show that there is a small number of distinct clusters in the posterior.
We can do this both for the unperturbed posterior $\pi \otimes \Pi$ and the perturbed posterior $\pi \otimes \Pi_{\frac{t}{\sqrt{n}}, \theta}$
We can rewrite the posterior using latent variables $Z_i$. 
Denote by $K_n$ the number of distinct values in $Z_i$.
We want this number to be much smaller than $\sqrt{n}$
\begin{assumption}
    \label{ass:SmallNumberClusters}
    We assume that for all $t$ in a neighbourhood of $0$, and for $U$ a neighbourhood of $\theta_0$, 
    \[
        \pi \otimes \Pi_{ \frac{t}{\sqrt{n}}, \theta} \left( \theta + \frac{t}{\sqrt{n}} \not\in U, K_n \geq k_n \given X^{(n)} \right) = o(1),
    \]
    for some sequence $k_n = o(\sqrt{n})$.
\end{assumption}
To verify \Cref{ass:SmallNumberClusters} we can either use a direct argument, or use the remaining mass theorem \cite[Theorem 8.20]{ghosalFundamentalsNonparametricBayesian2017}.
We provide a suitable tail bound on the distinct number of clusters under the Dirichlet process prior in \Cref{lem:tailbound_distinct_obs_DP}.
For a Mixture of finite mixtures, the number of clusters is given by $K$, so all that is needed is to show that $\PP(K > k_n)$ is small enough.

Finally, we need to assume the following consistency result
\begin{assumption}
    \label{ass:Consistency}
    Assume that for all $t$ the following limit converges to $1$.
    \[
\frac{
    \iint_{\Theta_n, \mathcal{F}_n} e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{\frac{t}{\sqrt{n}}}(\theta, F)\right)} \dd \pi(\theta) \dd \Pi(F)
    }{
        \iint e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{\frac{t}{\sqrt{n}}}(\theta, F)\right)} \dd \pi(\theta) \dd \Pi(F)
    }
    \rightsquigarrow 1.
    \] 
\end{assumption}

With these assumptions, we can prove the lemma that will allow us to verify the chance of measures condition. 
\begin{lem}\label{lem:ChangeOfMeasure}
    Let $\Pi$ be a a species sampling process with center measure $G$, such that $G$ has density $g$.
    Let $\pi$ be be a probability distribution on $\Theta$ with density $h$.  
    Suppose that for all $t \in T$, with $T$ a open neighbourhood of $0$ \Cref{ass:ChangeOfVariables,ass:Smoothness,ass:SmallNumberClusters} hold.
        Then
    \[
        \frac{
            \iint_{\Theta_n, \mathcal{F}_n} e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{\frac{t}{\sqrt{n}}}(\theta, F)\right)} \dd \pi(\theta) \dd \Pi(F)
        }{
            \iint_{\Theta_n, \mathcal{F}_n} e^{\ell_n\left(\theta, F\right)} \dd \pi(\theta) \dd \Pi(F)
        }
        \rightsquigarrow 1.  
    \]
\end{lem}

\begin{proof}
    First, by \Cref{ass:Consistency} it suffices to show
        \[
        \frac{
            \iint e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{\frac{t}{\sqrt{n}}}(\theta, F)\right)} \dd \pi(\theta) \dd \Pi(F)
        }{
            \iint e^{\ell_n\left(\theta, F\right)} \dd \pi(\theta) \dd \Pi(F)
        }
        \rightsquigarrow 1.  
    \]

    By \Cref{ass:SmallNumberClusters} we see that 
    \begin{align*}
        &\int_{U + \frac{t}{\sqrt{n}}} \int_{K \leq k_n} e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{t/\sqrt{n}}(\theta, F) \right)} \dd \Pi(F) \dd \pi(\theta) \\
        &\sim \iint e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{t/\sqrt{n}}(\theta, F) \right)} \dd \Pi(F) \dd \pi(\theta).
    \end{align*}
    By evaluating this when $t = t$ and $t = 0$, we find that
    \begin{align*}
      & \frac{
          \iint e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{t/\sqrt{n}}(\theta, F) \right)} \dd \Pi(F) \dd \pi(\theta)
      }{
        \iint e^{\ell_n\left(\theta, F \right)} \dd \Pi(F) \dd \pi(\theta)
      }\\
      &\sim \frac{
          \int_{U + \frac{t}{\sqrt{n}}} \int_{K \leq k_n} e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{t/\sqrt{n}}(\theta, F) \right)} \dd \Pi(F) \dd \pi(\theta) 
      }{
        \int_U \int_{K \leq k_n} e^{\ell_n\left(\theta, F \right)} \dd \Pi(F) \dd \pi(\theta)
    }.
    \end{align*}
    In the integral in the numerator we do a change of variables $\theta + \frac{t}{\sqrt{n}} \mapsto \theta$.
    \begin{align*}
       &\int_{U + \frac{t}{\sqrt{n}}} \int_{K \leq k_n} e^{\ell_n\left(\theta + \frac{t}{\sqrt{n}}, F_{t/\sqrt{n}}(\theta, F) \right)} \dd \Pi(F) \dd \pi(\theta) 
      \\
      & =\int_{U} \int_{K \leq k_n} e^{\ell_n\left(\theta, F_{t/\sqrt{n}}(\theta - \frac{t}{\sqrt{n}}, F) \right)} \dd \Pi(F) h(\theta - \frac{t}{\sqrt{n}}) \dd \theta 
  \end{align*}
  By \Cref{ass:smoothnessinh} in \Cref{ass:Smoothness} and \Cref{lem:MoveRatioBoundIntoSum} we find that 
  \[
      \left\|
      \frac{
          \int_{U} \int_{K \leq k_n} e^{\ell_n\left(\theta, F_{t/\sqrt{n}}(\theta - \frac{t}{\sqrt{n}}, F) \right)} \dd \Pi(F) h(\theta - \frac{t}{\sqrt{n}}) \dd \theta
      }{
          \int_U \int_{K \leq k_n} e^{\ell_n\left(\theta, F \right)} \dd \Pi(F) h(\theta) \dd \theta
      } - 1
      \right\| \leq \frac{c_t}{\sqrt{n}}
  \]
  By \Cref{ass:ChangeOfVariables} and \Cref{lem:ChineseRepSpeciesSampling}, it follows that 
    \begin{align*}
        &\int_{K \leq k_n} e^{\ell_n\left(\theta , F_{t/\sqrt{n}}(\theta - \frac{t}{\sqrt{n}}, F) \right)} \dd \Pi(F) \\
        &=  \sum_{\mathcal{S} \in S(n)} \II_{\# \mathcal{S} < k_n} \mathcal{P}(S) \prod_{i = 1}^{\#\mathcal{S}} \int \prod_{j \in S_i} p_{\theta}(X_j\given \phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \dd G(z),
    \end{align*}
    where $S(N)$ is the collection of partitions of $[n]$.
    By plugging this in the preceeding expression we get
    \begin{align*}
        \frac{
            \sum_{\mathcal{S} \in S(n)} \II_{\# \mathcal{S} < k_n} \mathcal{P}(S) \int_{U} \prod_{i = 1}^{\#\mathcal{S}} \left[\int \prod_{j \in S_i} p_{\theta }(X_j\given \phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \dd G(z)\right] \dd \pi(\theta) 
      }{
          \sum_{\mathcal{S} \in S(n)} \II_{\# \mathcal{S} < k_n} \mathcal{P}(S) \int_U \prod_{i = 1}^{\#\mathcal{S}} \left[\int \prod_{j \in S_i} p_{\theta}(X_j\given z) \dd G(z) \right] \dd \pi(\theta)
    }.
    \end{align*}

    We will now apply the change of variables $\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z) \mapsto z$. 
    We will study the effect in steps. 
    We start by analysing
    \begin{align*}
        &\frac{\int \prod_{j \in S_i} p_{\theta}(X_j\given \phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \dd G(z)}{\int \prod_{j \in S_i} p_{\theta}(X_j\given z) \dd G(z)} \\
        &=\frac{\int \prod_{j \in S_i} p_{\theta }(X_j\given z) g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}( z)) \|\det \dot \phi^{-1}_{t, \theta - \frac{t}{\sqrt{n}}} \| \dd z}{\int \prod_{j \in S_i} p_{\theta}(X_j\given z) g(z) \dd z} 
    \end{align*} 
    By using \Cref{ass:smoothnessinG} of \Cref{ass:Smoothness} and \Cref{lem:MoveRatioBoundIntoSum} we see that uniformly for all $\theta \in U$ and every partition $S \in S(n)$ and every $S_i \in S$
    \[
        \left\| \frac{\int \prod_{j \in S_i} p_{\theta }(X_j\given z) g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}( z)) \|\det \dot \phi^{-1}_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}} \| \dd z}{\int \prod_{j \in S_i} p_{\theta}(X_j\given z) g(z) \dd z} 
        - 1 \right\| \leq \frac{C_t}{\sqrt{n}}.
    \]
    Next we use that when $\| \frac{a_i}{b_i} - 1 \| \leq \frac{C_t}{\sqrt{n}}$, then $\| \log \left( \frac{a_i}{b_i} \right) \| = \| \log \left( 1 + \frac{ a_i - b_i}{b_i} \right) \| \leq \|\frac{a_i}{b_i} - 1\|$. Hence $\| \log \prod_{i = 1}^{k_n} \left( \frac{a_i}{b_i} \right) \| \leq \sum_{i = 1}^{k_n} \| \log \frac{a_i}{b_i} \| \leq \frac{C_t k_n}{\sqrt{n}} \rightarrow 0$. By continuity of the exponential map, then also $\| \prod_{i = 1}^{k_n} \frac{a_i}{b_i} - 1 \| \rightarrow 0$ uniformly.
    This yields that uniformly for every partition $S \in S(n)$ with $\# S < k_n = o(\sqrt{n})$ and $\theta \in U$, 
    \[
        \left\| \frac{ \prod_{i = 1}^{\# S} \left[ \int \prod_{j \in S_i} p_{\theta }(X_j\given z) g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}( z)) \|\det \dot \phi^{-1}_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}} \| \dd z  \right]}{ \prod_{i = 1}^{\# S} \left[ \int \prod_{j \in S_i} p_{\theta}(X_j\given z) g(z) \dd z \right] } - 1 \right\| \rightarrow 0.
    \]
    Hence also when we sum over all such partitions in the numerator and denominator. 
    \[
        \left\|
        \frac{
            \int_{K \leq k_n} e^{\ell_{\theta, F_{\frac{t}{\sqrt{n}}}}\left( \theta, F_{\frac{t}{\sqrt{n}}}(\theta - \frac{t}{\sqrt{n}}, F) \right)} \dd \Pi(F)
        }{
            \int_{K \leq k_n} e^{\ell_{\theta, F}} \dd \Pi(F)
        } - 1
        \right\| \rightarrow 0,
    \]
    uniformly in $\theta \in U$ as $n \rightarrow \infty$.
    Finally plugging this in the previous result combined with \Cref{lem:MoveRatioBoundIntoSum} we get the final result.
\end{proof}

\textbf{Supporting Lemma}
Our first lemma is used to characterise expectations of products of functions of observations of a species sampling process.
In our paper, we plug in the likelihood and use a latent variable representation.
\begin{lem}\label{lem:ChineseRepSpeciesSampling}
    Let $\Pi$ be a species sampling prior with EPPF $\mathcal{P}$ and center measure $G$. 
    If we sample $Z_1,\dots, Z_n \given P \sim P$ for $P \sim \pi$, we have
    \[
        \EE[ \prod_{i = 1}^n f_i(Z_i)] = \sum_{\mathcal{S} \textrm{Partition of }[n]} \mathcal{P}(S) \prod_{i = 1}^{\#\mathcal{S}} \int \prod_{j \in S_i} f_{j}(z) \dd G(z).
    \]
\end{lem}

\begin{proof}
    The probability that a random partition $\mathcal{S}$ takes value $S$ is given by the EPPF $\mathcal{P}$, $\mathcal{P}(S)$.
    Given a partition $\mathcal{S} = S$, we can compute the conditional probability by splitting the data into each of the $K_n$ partitions, and then integrating out using the center measure $G$.
    This yields
    \begin{align*}
        \EE[ \prod_{i = 1}^n f_i (Z_i)] &= \EE[ \EE[ \prod_{i = 1}^n f_i (Z_i) | \mathcal{S} = S]] \\
            &= \EE[ \EE[ \prod_{i = 1}^{K_n} \prod_{j \in S_i} f_i (\theta_i)|\mathcal{S} = s ] ]\\
            &= \EE[ \EE[ \prod_{i = 1}^{K_n} \int \prod_{j \in S_i} f_i (\theta) \dd G(\theta) | \mathcal{S} = S]]\\
            &= \EE[ \prod_{i = 1}^{K_n} \int \prod_{j \in S_i} f_i (\theta) \dd G(\theta) ] \\
            &= \sum_{S \textrm{ Partition of }[n]} \mathcal{P}(S) \prod_{i = 1}^{K_n} \int \prod_{j \in S_i} f_i (\theta) \dd G(\theta)
    \end{align*}
\end{proof}

To show \Cref{ass:Smoothness} might require a specific argument for \Cref{ass:smoothnessinG}.
In our examples, we can use the following lemma:
\begin{lem}
    \label{lem:SmoothnessInG}
    Suppose that there exists a neighbourhood $U$ of $\theta_0$ such that there exists constants $L, L', C, C'> 0 $ such that
    \begin{align*}
        \|\det \dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - 1 \| & \leq C \frac{t}{\sqrt{n}}\\
        \| \frac{g(\phi_{\frac{t}{\sqrt{n}},\theta - \frac{t}{\sqrt{n}}}(z)) - g(z)}{g(z)}\| &\leq L' \frac{t}{\sqrt{n}}
    \end{align*}
    for all $\theta \in U$, $z$ and $x$ small enough.
    Then \Cref{ass:smoothnessinG} is satisfied.
\end{lem}

The conditions of this lemma seem somewhat natural, the change of variables $\phi_t$ has to converge to the identity, cannot have unbounded derrivatives and $g$ has to be locally Lipschitz in a suitable way.
\begin{proof}
    First we can use the triangle inequality to get
    \[
        \|\det \dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1}\| \leq \|\det \dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - 1\| + 1 \leq C \frac{t}{\sqrt{n}} + 1 \leq L, 
    \]
    by bounding for $n = 1$, setting $L = Ct + 1$.
    To show \Cref{ass:smoothnessinG} we will use the triangle inequality and the assumptions as follows
    \begin{align*}
        &\left\| \frac{g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{sqrt{n}}}(z)) \det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1}}{g(z)} -1 \right\| \\
        &=  \left\| \frac{g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - g(z)}{g(z)} \right\|\\
        &=  \left\| \frac{g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) \det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - g(z) \det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1}}{g(z)}\right\|\\
        &+ \left\|\frac{g(z)\det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - g(z)}{g(z)} \right\| \\
        &  \leq \left\|\det\dot \phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} \right\| \left\| \frac{g(\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)) - g(z)}{g(z)} \right\| \\
        &+ \left\|\det\dot\phi_{\frac{t}{\sqrt{n}}, \theta - \frac{t}{\sqrt{n}}}(z)^{-1} - 1 \right\| \\
    &\leq ( L L' + C) \frac{t}{\sqrt{n}}
    \end{align*}
\end{proof}

To verify \Cref{ass:smoothnessinh} we can use the following result
\begin{lem}
    \label{lem:SmoothnessInH}
    Suppose that the prior density $h$ is continuously differentiable and nonzero in a neighbourhood of $\theta_0$. Then there exists a neighbourhood $U$ and $C_t$ such that, for all $n$ large enough
    \[
         \| \frac{h( \theta + \frac{t}{\sqrt{n}})}{h(\theta)} - 1 \| \leq \frac{C'_T}{\sqrt{n}}
    \]
    for all $\theta \in U$.
\end{lem}

\begin{proof}
    Because $h$ is continuously differentiable in a neighbourhood of $\theta_0$, it is locally Lipschitz in a neighbourhood of $\theta_0$. Call this constant $L$. Then
    \begin{align*}
        \| \frac{ h( \theta + x)}{h(\theta)} - 1 \| &= \| \frac{ h(\theta + x) - h(\theta)}{h(\theta)} \| \\
        & = \frac{ \| h(\theta + x) - h(\theta) \|}{ h(\theta)} \\
        & \leq \frac{ L}{\inf_{\theta in U} h(\theta)} x
    \end{align*}
    provided that $x$ is close to $0$.
    For $n$ large enough $\frac{t}{\sqrt{n}}$ will be close to $0$.
\end{proof}

\begin{lem}\label{lem:MoveRatioBoundIntoSum}
    If $\nu$ is a measure and suppose that two sequences of nonnegative functions satisfy the relation $f_n, g_n$$\sup_x \| \frac{g_n(x)}{f_n(x)} - 1 \| \rightarrow 0$, then
    \[
        \left\|
        \frac{\int g_n(x) \dd \nu(x)}{\int f_n(x) \dd \nu(x)} - 1
        \right\| \rightarrow 0
    \]
\end{lem}

\begin{proof}
    \begin{align*}
        \left\|
        \frac{\int g_n(x) \dd \nu(x)}{\int f_n(x) \dd \nu(x)} - 1
        \right\| &=  \left\|
        \frac{\int g_n(x) - f_n(x) \dd \nu(x)}{\int f_n(x) \dd \nu(x)}
        \right\|\\
        &\leq 
        \frac{\int \| g_n(x) - f_n(x) \| \dd \nu(x)}{\int f_n(x) \dd \nu(x)}\\
        &=\frac{\int f_n(x) \| \frac{g_n(x) - f_n(x)}{f_n(x)} \| \dd \nu(x)}{\int f_n(x) \dd \nu(x)} \\
        &\leq \frac{\int f_n(x) \sup_y \left \|\frac{g_n(y)}{f_n(y)} - 1 \right\| \dd \nu(x)}{\int f_n(x) \dd \nu(x)}\\
        &=  \sup_y \left \|\frac{g_n(y)}{f_n(y)} - 1 \right\| \rightarrow 0.
    \end{align*}
\end{proof}<++>


==> oldstuff/Semiparametricbvm.tex <==
\section{Semiparametric Bernstein-von Mises Theorem}\label{sec:semiparBvM}
Let $X_1,\ldots, X_n$ be an i.i.d.\ sample from a density $p_{\q,F}$ relative to a $\s$-finite measure on 
a measurable space $(\X,\A)$, for parameters $\q\in\Theta\subset\RR^d$ and $F$ ranging over a set $\F$, equipped
with a $\s$-field. Let $\ell_n(\q,F)=\log \prodin p_{\q,F}(X_i)$ be the log likelihood.
Given a prior $\Pi$ on $\Theta\times\F$, a posterior distribution of $(\q,F)$ given $X_1,\ldots, X_n$ is defined,
by Bayes's formula, as 
$$\Pi_n\bigl((\q,F)\in B\given X_1,\ldots,X_n\bigr)=\frac{\int_B e^{\ell_n(\q,F)}\,d\Pi(\q,F)}{\int e^{\ell_n(\q,F)}\,d\Pi(\q,F)}.$$
We are interested in proving a Bernstein-von Mises type theorem for
the marginal posterior distribution of $\q$.
This theorem gives a normal approximation with centering and covariance determined by the efficient
influence function for estimating $\q$. However, the following theorem is stated in abstract terms. We interpret
the objects involved and its conditions after the proof. The theorem can be considered a version of
Theorem~2.1 in \cite{castilloBernsteinMisesTheorem2015} for estimating the parameter of a semiparametric model.
It measures the discrepancy between the posterior distribution and its normal approximation through the
weak topology rather than the much stronger total variation distance, as in \cite{castilloSemiparametricBernsteinMises2012}, but
under weaker conditions on the prior distribution.

Let $\tilde\ell_0:\X\to \RR^d$ be a measurable map such that $P_0\tilde\ell_0=0$ and such that the matrix
$\tilde I_0:=\Cov_0\bigl(\tilde\ell_0(X_1)\bigr)$ exists and is nonsingular. The subscript $0$ will later be
taken to refer to the true parameter $(\q_0, F_0)$, but does not have a special meaning in the abstract theorem.
Let $\PP_n$ denote the empirical measure of  $X_1,\ldots, X_n$
and $\ep_n=\sqrt n(\PP_n-P_0)$ the empirical process with centering $P_0$.

For given $(\q,F)\in \Theta\times\F$, assume that there exists a map $t\mapsto F_t(\q,F)$ from a given neighbourhood of
$0\in\RR^d$ to $\F$ such that, for given measurable subsets $\Theta_n\subset \Theta$ and $\F_n\subset\F$,
\begin{align*}
&\ell_n\Bigl(\q+\frac t{\sqrt n},F_{t/\sqrt n}(\q,F)\Bigr)-\ell_n(\q,F)\\
&\qquad\qquad=t^T\GG_n\tilde\ell_0-t^T\bigl(\tilde I_0+R_{n,1}(\q,F)\bigr)\sqrt n(\q-\q_0)
 -\thalf t^T\tilde I_0 t+R_{n,2}(\q,F),
\end{align*}
for a matrix-valued process $R_{n,1}$ and and scalar process $R_{n,2}$ such that 
\begin{align}
\label{EqRemainders}
&\sup_{\q\in\Theta_n,F\in\F_n}\bigl\| R_{n,1}(\q,F)\bigr\|+|R_{n,2}(\q,F)|\stackrel {P_0^n}\longrightarrow 0,
\end{align}
and such that
\begin{align}
\label{EqChangeOfMeasure}
\frac{\int_{\Theta_n\times \F_n} e^{\ell_n\bigl(\q-t/\sqrt n,F_{-t/\sqrt n}(\q,F)\bigr)}\,d\Pi(\q,F)}
{\int_{\Theta_n\times \F_n}  e^{\ell_n(\q,F)}\,d\Pi(\q,F)} \stackrel {P_0^n}\longrightarrow 1.
\end{align}

Let $\mathrm{BL}_1$ be the set of all functions $h: \RR^d\ra [0,1]$ such that $|h(x)-h(y)|\le \|x-y\|$, for every $x,y\in\RR^d$.

\begin{thm}\label{thm:semiparametricBvM}
If $\Pi_n(\q\in \Theta_n, F\in\F_n\given X_1,\ldots, X_n)\ra 1$, in $P_0^n$-probability, and \eqref{EqRemainders}-\eqref{EqChangeOfMeasure}
hold, then
$$\sup_{h\in \mathrm{BL}_1}\E \Bigl|h\bigl(\tilde I_0\sqrt n(\q-\q_0)-\ep_n\tilde\ell_0\bigr)-\int h\,dN(0,\tilde I_0)\Bigr|
\stackrel {P_0^n}\longrightarrow 0.$$
\end{thm}

\begin{proof}
The total variation distance between the posterior distribution relative to the given prior and the posterior distribution
relative to this prior conditioned to the set $\Theta_n\times \F_n$ is bounded by 
$\Pi_n\bigl((\q,F)\notin \Theta_n\times\F_n\given X_1,\ldots, X_n\bigr)$ (see e.g.\ Lemma~K.10 in 
\cite{ghosalFundamentalsNonparametricBayesian2017}), and hence tends to zero in probability, by assumption.
Thus we may assume that $\Pi(\Theta_n\times\F_n)=1$.

The Laplace transform of $V_n(\q,F):=\bigl(\tilde I_0+R_{n,1}(\q,F)\bigr)\sqrt n(\q-\q_0)-\ep_n\tilde\ell_0$ relative to the
posterior distribution of $(\q,F)$ given $X_1,\dots, X_n$ is given by
\begin{align*}
t\mapsto %\E \Bigl(e^{t^T\bigl(\tilde I_0+R_{n,1}(\q,F)\bigr)\sqrt n(\q-\q_0)-t^T\ep_n\tilde\ell_0}\given X_1,\ldots, X_n\Bigr)\\
\E \Bigl(e^{t^TV_n(\q,F)}\given X_1,\ldots, X_n\Bigr)
&=\frac{\int e^{t^TV_n(\q,F)}e^{\ell_n(\q,F)}\,d\Pi(\q,F)}{\int e^{\ell_n(\q,F)}\,d\Pi(\q,F)}\\
&=e^{t^T\tilde I_0t/2}\,\frac{\int e^{-R_{n,2}(\q,F)} e^{\ell_n(\q-t/\sqrt n,F_{-t/\sqrt n}(\q,F))}\,d\Pi(\q,F)}{\int e^{\ell_n(\q,F)}\,d\Pi(\q,F)},
\end{align*}
by the definitions of $R_{n,1}$ and $R_{n,2}$, for $n$ and $t$ such that $-t/\sqrt n$ is in the neighbourhood 
of $0$ where the perturbations $s\mapsto F_s(\q,F)$ are defined. 
Since $R_{n,2}(\q,F)\ra 0$, uniformly in $(\q,F)$, by \eqref{EqRemainders}, the factor $e^{-R_{n,2}(\q,F)}$ can be taken
out of the integral at the cost of a multiplicative $e^{o_P(1)}$-term. The remaining quotient of integrals 
tends in probability to 1 by \eqref{EqChangeOfMeasure}. Thus 
the right side of the display tends in probability to $e^{t^T\tilde I_0t/2}$, for every fixed $t$ in a neighbourhood of 0. The pointwise
convergence of Laplace transforms implies that $V_n(\q,F)\given X_1,\ldots,X_n\weak N(0,\tilde I_0)$
(e.g.\ \cite{raySemiparametricBayesianCausal2020}, Lemma~14, applied to linear combinations and Cram\'er-Wold device), i.e.
$$\sup_{h\in \mathrm{BL}_1}\E \Bigl|h\bigl(V_n(\q,F)\bigr)-\int h\,dN(0,\tilde I_0)\Bigr| \stackrel {P_0^n}\longrightarrow 0.$$
On the event
$A_n=\{\sup_{\q,F}\|\tilde I_0\bigr(\tilde I_0+R_{n,1}(\q,F)\bigr)^{-1}-I\|<\e\}$, we have
$$\bigl\|\tilde I_0\sqrt n(\q-\q_0)-\bigr(\tilde I_0+R_{n,1}(\q,F)\bigr)\sqrt n(\q-\q_0)\bigr\|
\le\e \bigl\|\bigr(\tilde I_0+R_{n,1}(\q,F)\bigr)\sqrt n(\q-\q_0)\bigr\|.$$
Hence for every $M$ and Lipschitz $h: \RR^d\ra[0,1]$,
\begin{align*}
&\Bigl|\E 1_{A_n}\Bigl(h\bigl(\tilde I_0\sqrt n(\q-\q_0)-\ep_n\tilde\ell_0\bigr)-h\bigl(V_n(\q,F)\bigr)\given X_1,\ldots,X_n\Bigr)\Bigr|\\
&\qquad\qquad\le \e M+\Pr\Bigl(\bigl\|V_n(\q,F)+\ep_n\tilde\ell_0\bigr\|>M\given X_1,\ldots, X_n\Bigr).
\end{align*}
Because there exists a Lipschitz function with $1_{\|v\|>M}\le h(v)\le 1_{\|v\|>M-1}$, the bounded Lipschitz metric is
invariant under location shifts, 
the second term is bounded above by $N\bigl(\ep_n\tilde\ell_0,\tilde I_0\bigr)\{v: \|v\|>M-1\}+o_P(1)$. It follows that
\begin{align*}
&\Bigl|\E \Bigl(h\bigl(\tilde I_0\sqrt n(\q-\q_0)-\ep_n\tilde\ell_0\bigr)\given X_1,\ldots,X_n\Bigr)-\int h\,dN(0,\tilde I_0)\Bigr| \\
&\qquad\le \Pr(A_n^c)+\e M+N\bigl(\ep_n\tilde\ell_0,\tilde I_0\bigr)\{v: \|v\|>M-1\}+o_P(1).
\end{align*}
The third and second terms on the right side can be made arbitrarily small by first choosing sufficiently large $M$, 
and next sufficiently small $\e$. For fixed $M$ and $\e$ the other terms tend to zero in probability. Hence
the left side tends to zero in probability, uniformly in $h$.
\end{proof}



In a typical application we construct the submodels $t\mapsto F_t(\q,F)$ to be least favourable at $(\q,F)$ for
estimating $\q$, i.e.\ 
the score function of the induced model $t\mapsto p_{\q+t,F_t(\q,F)}$ is the efficient score function at $(\q,F)$  for
estimating $\q$:
$$\frac{\partial}{\partial t}_{|t=0}\log p_{\q+t,F_t(\q,F)}(x)=\tilde\ell_{\q,F}.$$
Only the efficient score function at the true value $(\q_0,F_0)$ of the parameter enters the theorem.
This suggests some flexibility in the definition of the submodels, as has also been employed in 
proofs of semiparametric maximum likelihood (e.g.\ \cite{murphyProfileLikelihood2000}). The submodels need satisfy
the preceding display only approximately. \footnote{\color{red} They can also be made dependent on $n$?! Is that a
useful extension? Neyman-Scott might be a good test case.}

Condition \eqref{EqChangeOfMeasure} then requires that the prior does not change much 
``in the direction of the least favourable direction''. It is essential that the submodel extends in every
direction $t$ in a neighbourhood of 0, as this gives the asymptotic tightness of the posterior distribution,
by way of the Laplace transform employed in the proof of the theorem.



==> oldstuff/SymmetricLocationMixtures.tex <==
\section{Symmetric location mixtures}
Suppose that $p_\q(x\given z)=\phi\bigl((x-\q)/z\bigr)/z$, for a known smooth, symmetric density
$\phi$, for instance the standard normal density. Then the mixture is a symmetric 
density with mode $\q$. The model is adaptive and the least favourable
submodel is simply given by the parameters  $t\mapsto (\q+t,F)$.

Can this model already be dealt with by the methods in Ismael's first paper?
The change of measure in the direction of the least favourable model in $F$ is unnecessary,
makng the uniformity in $F$ the main challenge?



==> oldstuff/exponentialfrailty2.tex <==
\section{Exponential Frailty}

\subsection{LAN-expansion}
\input{FrailtyModelLikelihood.tex}
\subsection{Semiparametric verification}
The goal is to verify the Kullback-Leibler prior mass condition. 
We are going to give a strategy to give finite sample bounds.
So let us begin by making goal precise.
The Kullback-Leibler divergence between two densities $p_1, p_0$ with respect to a common dominating measure $\mu$ is defined to be
\[
    \text{KL}\left( p_0; p_1 \right) := \int p_0 \log( p_0/p_1) \dd \mu.
\]
The Kullback-Leibler variation is defined analogously to be
\[
    \text{V}_0\left( p_0; p_1 \right) := \int p_0 \left( \log(p_0/p_1) - \text{KL}\left( p_0; p_1 \right) \right)^2 \dd \mu
\]
We want to give bounds on sets Kullback-Leibler balls of the form
\[
    B_2( p_0, \epsilon)= \{ p : \text{KL}(p_0; p) \leq \epsilon^2, \text{V}_0(p_0, p) \leq \epsilon^2 \}
\]

In particular, we want to find a strategy to show this for dirichlet process mixtures. 
For sake of presentation, assume the true density is a mixture, however, only the approximation steps are needed, not existance of a true mixing distribution.
We will adopt this for sake of presentation.

Let $p_F$ be a mixture with density $x \mapsto \int p(x|z) \dd F(z)$.
Suppose the true density $p_0 = p_{F_0}$.
We put a Dirichlet process prior on $F$. 
Thus our goal becomes showing a bound on
\[
  \text{DP}\left( F: \text{KL}\left( p_{F_0}; p_F \right) \leq \epsilon^2, \text{V}_0\left( p_{F_0}; p_F \right) \leq \epsilon^2 \right)
\]

We will find a suitable subset $S_\epsilon$ such that for all $F \in S_\epsilon$ it holds that
\[
    \text{KL}\left( P_{F_0}; p_F \right) + \text{V}_0\left( P_{F_0}; P_F \right) \leq \epsilon
\]
If we can find a lower bound on
\[
    \text{DP}\left( S_\epsilon \right)
\]
then we are done.

So our next step is to find a suitable set $S_\epsilon$. 
The usual strategy works by finding another norm $\|\cdot \|$ and a $\delta = \delta_\epsilon$ such that if $\| p_{F_0} - p_{F} \| \leq \delta$ then 

    
\[
    \text{KL}\left( P_{F_0}; p_F \right) + \text{V}\left( P_{F_0}; P_F \right) \leq \epsilon^2.
\]

The usual strategy works by applying Lemma B.2 which allows to bound the Kullback-Leibler divergence and variation in terms of the Helling metric.
Note that this is not a trivial bound, however, it can be fixed in certain situations. 
A further note is that the $\text{V}_2$ given there is $\text{KL} + \text{V}_0$ in our case.

Then we can further bound the Helling metric by the $L_1$ metric. 
This means that it is enough to bound the prior mass if sets such that the miximg distribution is close in $L^1$ distance.

We could compare the $L^1$ distance between $p_{F}$ and $P_{F_0}$ and the $L^1$ distance on $F$ and $F_0$. 
Note that we are here using the explicit existance of mixtures, so in general we will not do this.

To continue, we aim to find a collection of finite measures $F = \sum_{i = 1}^{K_n} W_i\delta_{\theta_i}$ for some fixed (or bounded) $K_n$ with the following property
\[
  \| p_{F_0} - p_{F} \|_1 \leq \delta
\]

Our set $S_\epsilon$ will be these specific measures.
We will have to pick our locations $\theta_i$ in some nice subsets so we can give lower bounds on the prior probability.
This is the less trivial step.
The easier step is that we need to pick our weights $W_i$ in some intervals centred on a specific $w_i$ and with distance at most $\delta$.
We can control the prior was of this set by applying theorem G.13.

By using independence we can then give a lowerbound on our probability.

\subsection{Entropy computations}

\begin{lem}\label{lem:entropybound}
    Let $N_\epsilon, \underline{m}_\epsilon, \overline{m}_\epsilon$ as in  \Cref{lem:priormassbound}.
    Define   
    \begin{align*}
        \mathcal{P}_{\epsilon,1} := \{ \sum_i w_i \theta z_i^2 e^{-z_i ( x + \theta y)}&: \sum_{j > N_\epsilon} w_j < \epsilon, z_j \in [\underline{m}_\epsilon, \overline{M}_\epsilon], j = 1, \dots, N, \\& \qquad \theta \in [ \theta_0 \epsilon, \frac{\theta_0}{\epsilon}] \}.
    \end{align*}
    Then

    \[
        \log N(\epsilon, \mathcal{P}_\epsilon, \| \cdot \|_1) \lesssim N_\epsilon \log \left( \frac{1}{\epsilon} \right).
    \]
\end{lem}

\begin{proof}
    We first recall the definitions of $N_\epsilon, \underline{m}_\epsilon$ and $\overline{m}_\epsilon$ from  \Cref{lem:priormassbound}. That is
    \begin{align*}
        N_\epsilon &\sim C' \log \left(\frac{1}{\epsilon} \right)^2,\\ 
        \underline{m}_\epsilon &=  \frac{1}{\EE[Z^{-\gamma}]^{1/\gamma}} \epsilon^{-1/\gamma}, \\
        \overline{m}_\epsilon &=  \EE[Z^\gamma]^{1/\gamma} \epsilon^{1/\gamma}
    \end{align*}
    To cover $\{ (w_1, \dots, W_{N_\epsilon}): \sum_i w_i \leq 1 \}$ by an $\epsilon$-grid, we need by \cite[Proposition C.1]{ghosalFundamentalsNonparametricBayesian2017a},
    \[
        \left(\frac{5}{\epsilon} \right)^{N_\epsilon}
    \]
    Note that there exists a $C > 0$ such that 
    \[
        \| p_{\theta}(x,y \given z) - p_{\theta}(x,y \given w \|_1 \leq \frac{C}{\underline{m}_\epsilon} | z - w|
    \]
    By \Cref{lem:TVExponentials}, and since the total variation distance between products of independent random variables is less than the sum of the individual total variations, we find that $\| p_\theta(x,y \given z) - p_{\theta}(x,y \given w) \leq \frac{2 \| z - w \|}{w}$.
    We can give an upper bound for this by taking $ \frac{1}{w}$ to be the largest possible value, $\frac{1}{\underline{m}_\epsilon}$.
    If we put an $\frac{\underline{m}_\epsilon}{C} \epsilon $ grid on $[\underline{m}_\epsilon, \overline{m}_\epsilon]$ we get an $\| \cdot \|_1$ $\epsilon$ cover. \TODO{Give some more details maybe?!}
    Similarly for $[ \theta_0 \epsilon, \frac{\theta_0}{\epsilon}]$. We need $\epsilon^2$ points to cover in the $\| \cdot \|_1$ metric.
    This yields
    \[
        N(\epsilon, \mathcal{P}_\epsilon, \| \cdot \|_1 ) \leq \left( \frac{5}{\epsilon} \right)^{N_\epsilon} \times \left( \frac{\overline{m}_\epsilon}{\underline{m}_\epsilon \epsilon} \right)^{N_\epsilon} \times \frac{1}{\epsilon^2}.
    \]
    Hence $\log N(\epsilon, \mathcal{P}_\epsilon, \| \cdot \|_1) \lesssim N_\epsilon \log \left( \frac{1}{\epsilon} \right)$.
\end{proof}

\begin{lem}\label{lem:Sievepriormass}
    In the notation of \Cref{lem:entropybound}. 
    Suppose that $G$ is a probability distribution such that $G([\underline{m}_\epsilon, \overline{m}_\epsilon]^c) \lesssim \epsilon^\beta$ for some $\beta > 0$.
    Suppose that $\pi\left( [ \theta_0 \epsilon, \frac{\theta_0}{\epsilon}]^c\right) \leq \epsilon^\beta$.
    Then
    \[
        \Pi\left( \mathcal{P}_\epsilon^c  \right) \leq e^{-N_\epsilon} + (N_\epsilon + 1) \epsilon^\beta.
    \]
\end{lem}

\begin{proof}
    By the proof of \cite[Lemma 7.15]{ghosalFundamentalsNonparametricBayesian2017a}, we find
    \[
        \Pi\left( \mathcal{P}_\epsilon^c \right) \leq \PP( \sum_{j \geq N_\epsilon} w_j \geq \epsilon ) + N G([\underline{m}_\epsilon, \overline{m}_\epsilon] + \pi\left( [ \theta_0 \epsilon, \frac{\theta_0}{\epsilon}]^c\right).
    \]
    Per our assumptions, the latter two are less than $N_\epsilon \epsilon^\beta$ and $\epsilon^\beta$ respectively.
    By the proof of \cite[Lemma 7.15]{ghosalFundamentalsNonparametricBayesian2017a} we find that
    \[
        \PP( \sum_{j \geq N_\epsilon} w_j \geq \epsilon ) \leq e^{- N_\epsilon}
    \]
    Adding it all up gives the result.
\end{proof}

Now we can find optimal choices for $\epsilon_n$.
\begin{lem}
    If $e = \epsilon_n = \frac{ \log\left( n \right)^2}{\sqrt{n}}$ we find, for $n$ large enough
    \begin{align*}
        \log N(\epsilon, \mathcal{P}_\epsilon, \| \cdot \|_1) &\leq n \epsilon_n^2\\
        \Pi\left( \mathcal{P}_\epsilon^c  \right) &\leq = o(e^{- \frac{\beta}{3} \log n}).
    \end{align*}
\end{lem}
\begin{proof}
    Note $n \epsilon_n^2 = \log(n)^4$ and $\log( \frac{1}{\epsilon_n}) \leq \frac{1}{2} \log(n)$. Pick $N_{\epsilon_n} \sim \log(n)^2$.
    By \Cref{lem:entropybound} and \Cref{lem:Sievepriormass} and algebra,
    \begin{align*}
        \log N(\epsilon, \mathcal{P}_\epsilon, \| \cdot \|_1) &\lesssim \log\left( n \right)^3 \leq n \epsilon_n^2\\
        \Pi\left( \mathcal{P}_\epsilon^c  \right) &\leq e^{-\log(n)^2} + (\log(n)^2 + 1) \left(\frac{\log(n)^2 }{\sqrt{n}} \right)^\beta = o(e^{- \frac{\beta}{3} \log n}).
    \end{align*}
\end{proof}
If we pick $\overline{\epsilon}_n = \sqrt{ \frac{\log(n)}{3n} }$ we can apply the remaining mass theorem \cite[Theorem 8.20]{ghosalFundamentalsNonparametricBayesian2017a}.

\subsection{Contraction rates}

Idea: Measure distance in $F$ by the Wasserstein metric, euclidean metric on $\theta$. \\
This should give contraction rates for $(\theta, F)$, and imply rates for $p_{\theta, F}$ in some useful metric.
Details are yet to be figured out.

\subsection{Bernstein-von Mises for $\theta$}
With everything set up, we can also prove a BvM type result for $\theta$. \TODO{redo the proof once 1) maximal inequality conditions are written up, 2) Contraction rates are done, and 3) once \Cref{lem:ChangeOfMeasure} is rewritten}.
\begin{thm}
    In the model $(X_i, Y_i)\given \theta, F \overset{i.i.d.}\sim P_{\theta, F}$, in the frailty model.
    Suppose $\theta \sim \pi$ and $F \sim \textrm{DP}(MG)$.
    Suppose $G$ has a density $g$ with $g(z) \gtrsim \left( \frac{1}{1 + z} \right)^\alpha$.
    Suppose $\pi$ admits a density $h$ which is nonzero and differentiable in $\theta_0$.
    Then
    \[
        \sup_{h\in \mathrm{BL}_1}\E \Bigl|h\bigl(\tilde I_0\sqrt n(\q-\q_0)-\ep_n\tilde\ell_0\bigr)-\int h\,dN(0,\tilde I_0)\Bigr|
\stackrel {P_0^n}\longrightarrow 0.
    \]
\end{thm}

\begin{proof}
    In order to apply \Cref{thm:semiparametricBvM} we need to verify \Cref{EqRemainders,EqChangeOfMeasure}.
    The least favourable submodel in the frailty model is 
    \[
        F_t(B) = F\left( B\left( \frac{2 \theta}{2 \theta - t} \right)\right).
    \]
    \textbf{Verifying the likelihood condition \eqref{EqRemainders}}\\
    \TODO{Check \Cref{EqRemainders} by maximal inequalities}.\\
    \textbf{Verifying the change of measure condition \eqref{EqChangeOfMeasure}}\\
    We want to apply \Cref{lem:ChangeOfMeasure}.
    For all $t$ the perturbed models are consistent for estimating $\theta_0$ by \TODO{finish, either rate or consistency theorem, see what works best}.
    To verify the prior mass condition in \Cref{lem:ChangeOfMeasure} we apply \Cref{lem:priormassbound}. 
    This means we can apply \Cref{lem:ChangeOfMeasure}.
    This shows that \eqref{EqChangeOfMeasure} is satisfied.
\end{proof}

\subsection{Technical lemmas}


\begin{lem}\label{lem:BoundRatioIntegrals}
    Let $A_1,\dots, A_N$ be a partition of $\Omega$, $P, Q$ probability measures on $\Omega$ and let  $f, g : \Omega \rightarrow \RR_+$ be $P$, respectively $Q$, integrable functions. Then
    \[
        \frac{ \int f \dd P}{ \int g \dd Q} \leq \max_i \sup_{z, z' \in A_i} \frac{f(z)}{g(z')} \frac{P(A_i)}{Q(A_i)}.
    \]
\end{lem}

\begin{proof}
    Write $\int f \dd P = \sum_i \int_{A_i} f \dd P$, $\int g \dd Q = \sum_i \int_{A_i} g \dd Q$. Then
    \[
        \frac{ \int f \dd P}{ \int g \dd Q} = \frac{ \sum_i \int_{A_i} f \dd P}{ \sum_i \int_{A_i} g \dd Q } \leq \max_i \frac{ \int_{A_i} f \dd P}{ \int_{A_i} g \dd Q}.
    \]
    Note that
    \[
        \frac{ \int_{A_i} f \dd P}{ \int_{A_i} g \dd Q} \leq \frac{ \int_{A_i} \sup_{z \in A_i} f \dd P}{ \int_{A_i} \inf_{z' \in A_i} g(z') \dd Q} \leq \sup_{z, z'\in A_i} \frac{f(z)}{g(z')} \frac{ P(A_i)}{Q(A_i)}.
    \]
\end{proof}
The following argument was used before, but got replaced. The strategy itself might be useful for other kernels.
\begin{proof}
    \textbf{Step 3: bounding in $F$ component}
    Our goal is to apply \Cref{lem:BoundRatioIntegrals}. To do this, we first need to compute the supremum on each of the intervals, and then study the bound we get.\\
    \textbf{Step 3i: computing the sups}.
    Note that on every $A_i$ we have $\frac{ \max A_i - \min A_i}{\min A_i} < 2 \epsilon$, $\min A_i \leq z, z_i \leq \max A_i$.
    \begin{align}
        \sup_{z, z_i \in A_i} 
            \frac{ 
                z^4 \theta_0 e^{-2z (x + \theta_0 y)}
            }{
                z_i^2 \theta_0 e^{-z_i(x + \theta_0 y)}
            }
            &\leq
            \sup_{z, z_i \in A_i} \frac{z^4 \theta_0}{z_i^2 \theta} \label{zbound}\\
            &\times\sup_{z, z_i \in A_i} \frac{e^{-2zx}}{e^{-z_i x}} \label{xbound}\\
            &\times\sup_{z, z_i \in A_i} \frac{e^{-2z \theta_0 y}}{e^{-z \theta y}} \label{ybound}
    \end{align}
    To bound \Cref{zbound} we observe that on $A_i$ $\min A_i < z_i, z < \max A_i < (1 + \epsilon) \min A_i$. Moreover, we assume that $\| \theta - \theta_0 \| \leq \epsilon \theta_0$, hence $\frac{\theta_0^2}{\theta} < \frac{1}{1 - \epsilon} \theta_0$. Thus, we can bound this by
    \[
         \sup_{z, z_i \in A_i} \frac{z^4 \theta_0}{z_i^2 \theta} \leq \left(1 + \epsilon\right)^4 \min A_i ^2 \frac{1}{1 - \epsilon} \theta_0.
    \]
    To bound \Cref{xbound}, we use that logarithms are increasing functions to see that we need to maximise $-(2zx - z_i x)$, this can be done by setting $z = \min A_i$ and $z_i = \max A_i$, which leads to the bound
    \[
        \sup_{z, z_i \in A_i} \frac{e^{-2zx}}{e^{-z_i x}} \leq e^{ (\max A_i - 2 \min A_i ) x} \leq e^{ (\epsilon - 1) \min A_i x}.
    \]
    Finally, to bound \Cref{ybound} we again use logarithms and pick the most extreme choices for $z, z_i$ and $\theta$. This leads to $\theta = (1 + \epsilon) \theta_0$, $z = \min A_i$ and $z_i = \max A_i$. This in turn gives us the bound 
    \[
        \sup_{z, z_i \in A_i} \frac{e^{-2z \theta_0 y}}{e^{-z \theta y}} \leq e^{-( 2 \min A_i \theta_0 - \max A_i (1 + \epsilon) \theta_0)y} \leq e^{-(2 - (1 + \epsilon)^2 ) \min A_i \theta_0 y}.
    \]
    Taking this all together leads to
    \[
         \sup_{z, z_i \in A_i} 
            \frac{ 
                z^4 \theta_0 e^{-2z (x + \theta_0 y)}
            }{
                z_i^2 \theta_0 e^{-z_i(x + \theta_0 y)}
            }
        \leq B_i(x,y),
    \]
    where $B_i(x,y)$ is given by
    \[
        B_i(x,y) =  \left(1 + \epsilon\right)^4 \min A_i ^2 \frac{1}{1 - \epsilon} \theta_0   e^{ (\epsilon - 1) \min A_i x} e^{-(2 - (1 + \epsilon)^2 ) \min A_i \theta_0 y}.
    \]
    
    By applying \Cref{lem:BoundRatioIntegrals} we can use this to bound the ratio of integrals by
    \[
        \frac{ \int p_{\theta_0}(x,y | z)^2 \dd F_0(z)}{ \int p_{\theta}(x,y | z) \dd F(z)} \leq \max_i B_i(x,y) \frac{F_0(A_i)}{w_i} \leq \sum_i B_i(x,y) \frac{F_0(A_i)}{w_i}.
    \]
    \textbf{Step 3ii: computing the integral of the bound}
    We now need to compute
    \[
        \int \int \sum_i B_i(x,y) \frac{F_0(A_i)}{w_i} \dd x \dd y.
    \]
    For each $B_i(x,y)$ we get
    \begin{align*}
        \int \int B_i(x,y) \dd x \dd y &=  \left(1 + \epsilon\right)^4 \min A_i ^2 \frac{1}{1 - \epsilon} \theta_0  \int e^{ (\epsilon - 1) \min A_i x} \dd x \int e^{-(2 - (1 + \epsilon)^2 ) \min A_i \theta_0 y} \dd y \\
        &=  \left(1 + \epsilon\right)^4 \min A_i ^2 \frac{1}{1 - \epsilon} \theta_0 \frac{1}{(\epsilon - 1) \min A_i} \frac{1}{-(2 - (1 + \epsilon)^2 ) \min A_i \theta_0}\\
        &= \frac{ \left( 1 + \epsilon \right)^4 }{ \left( 1 - \epsilon \right)^2 \left( 2 - \left(1 + \epsilon\right)^2 \right)}  
    \end{align*}
     If we plug this back in, we get
     \[
         \iint \sum_i B_i(x,y) \frac{ F_0(A_i)}{w_i} \dd x \dd y \leq  \frac{ \left( 1 + \epsilon \right)^4 }{ \left( 1 - \epsilon \right)^2 \left( 2 - \left(1 + \epsilon\right)^2 \right)} \sum_i \frac{F_0(A_i)}{w_i}.
     \]
     \textbf{Step 3iii: Bounding $ \sum_i \frac{F_0(A_i)}{w_i}$}.
     To bound $ \sum_i \frac{F_0(A_i)}{w_i}$ we use our assumption that $\min w_i > \frac{\epsilon^2}{2}$, and that $\sum_{i} F_0(A_i) \leq 1$. This yields
     \[
         \sum_i \frac{F(A_i)}{w_i} \leq \sum_i \frac{F(A_i)}{\min_j w_j} \leq \frac{2}{\epsilon^2}.
     \]
     This leads to the final bound 
     \[
         \iint
        \frac{
            \int_{A_0^c} p_{\theta_0}(x, y | z)^2 \dd F_0(z)
        }{
            \int p_{\theta}(x,y | z) \dd F(z)
        }
        \leq \frac{ \left( 1 + \epsilon \right)^4 }{ \left( 1 - \epsilon \right)^2 \left( 2 - \left(1 + \epsilon\right)^2 \right)} \frac{2}{\epsilon^2}
     \]

\end{proof}







==> oldstuff/introduction.tex <==
\section{Introduction}

Statistical modeling often involves striking a delicate balance between flexibility and simplicity. 
While parametric models offer a straightforward representation of data, they may fail to capture the intricate complexities present in real-world phenomena. 
On the other hand, nonparametric models provide remarkable flexibility but their complexity can also be a drawback.

Semiparametric modelling is a compromise that tries to combine the strengths of parametric and nonparametric models.
(Strict) semiparametric models incorporate both a flexible nonparametric component and a simpler parametric component.
Typically, the parameter of interest is part of the parametric component, and the suiscance parameters are part of the nonparametric components.

A mixture model is an example of a strict semiparametric model.
Mixture models are given by 3 objects:
\begin{enumerate}
  \item The kernel $p_{\theta} (x| z)$. A kernel gives for every $z$ a probability density. This kernel is known.
  \item A finite dimensional parameter of interest $\theta$, which is unknown.
  \item The nuisance parameter, a probability distribution $F$.
\end{enumerate}

The mixing distribution can then be defined with the density given by:
\begin{equation}
  p_{\theta, F}(x) = \int p_{\theta}(x | z) \dd F(z)\label{eq:mixingdensity}
\end{equation}

Equivalently, we can consider this as a latent variable model. 
We have some latent variable $Z \sim F$ that we do not observe, and the distribution of $X \given Z \sim p_\theta(x \given Z)$.
Because we do not observe $Z$, we might lose information for estimating $\theta$.
Semiparametric mixture models have a widespread application throughout statistics.
In this paper we will be considering three examples: symmetric location mixtures, exponential frailty and the errors-in-variables models.

Symmetric location mixtures 
\TODO{incorporate work of Jeanne}.
Exponential frailty models are a particular case of frailty models.
They are mixtures given by
\[
    p_{\theta, F}(x,y) = \int z^ 2 \theta e^{-z(x + \theta y)} \dd F(z)
\]
We will consider these examples in \Cref{sec:frailty}.
Semiparametric Bayesian frailty models have been considered in~\cite{walkerHierarchicalGeneralizedLinear1997,pennellBayesianSemiparametricDynamic2006,tallaritaBayesianAutoregressiveFrailty2020}.
A frequentist analysis of the semiparametric exponential frailty model with nonparametric maximum likelihood estimator has been done in~\cite{vandervaartEfficientMaximumLikelihood1996}.
See for examples of general frailty models~\cite{balanTutorialFrailtyModels2020}.

The errors-in-variables model is the last example we will consider. 
In this model we want to run a regression of $X$ on $Y$, however, we only observe noisy versions of $X$ and $Y$.
The mixture is given by
\[
    p_{\alpha, \beta, \sigma, \tau, F}(x,y) = \int \phi_\sigma(x - z) \phi_\tau(y - \alpha - \beta z) \dd F(z),
\]
where $\phi$ is the density of a standard normal Gaussian distribution.
For more details on the model see \Cref{sec:ErrorsInVars}.
Bayesian errors-in-variables have been considered before, see for example~\cite{dellaportasBayesianAnalysisErrorsinVariables1995,mallickSemiparametricErrorsinvariablesModels1996,mullerBayesianSemiparametricModel1997}.

The goal the statistician is to provide a reliable estimate for the parameter of inference $\theta$, and specify its uncertainty.
We want to learn $\theta$ as accurately as possible.
The first notion we need to guarantee is consistency, that is, the ability to find the true parameter at all.
After have esthablished consistency, we want to understand if our method is asymptotically optimal.

In the study of optimal statistical estimation, one key notion is the Fisher information.
In semiparametric statistics, we often deal with a loss of information and have to consider the efficient Fisher information.
We call a model differentiable in quadratic mean at $\theta_0$ if
\[
    \int \left[ \sqrt{p_\theta} - \sqrt{p_{\theta_0}} - \frac{1}{2} \dot\ell_{\theta_0} \sqrt{p_{\theta_0}} \right]^2 \dd \mu = o(\| \theta - \theta_0 \|),
\]
as $\theta \rightarrow \theta_0$. 
The Fisher information then is given by $I_{\theta_0} = P_{\theta_0} \dot\ell_{\theta_0}\dot\ell_{\theta_0}^T$.
Our goal is to prove that certain estimators are optimal.
To do so, we must first esthablish a lowerbound on how accurate estimators can be.
For this we use two ingredients,  Anderson's lemma~\cite[Lemma 8.5]{vandervaartAsymptoticStatistics1998} and The Convolution theorem~\cite[Lemma 8.8]{vandervaartAsymptoticStatistics1998}.
Let $l$ be a bowl-shaped loss-function, and $T_n$ a sequence of regular estimators.
By the convolution theorem

\[
    \sqrt{n}\left(T_n - \theta_0 \right) \rightsquigarrow N(0, I_{\theta_0}^{-1} ) \ast M_{\theta_0}.
\]
Then by Anderson's lemma
\[
    \int l \dd N(0, I_{\theta_0}) \ast M_{\theta_0} \geq \int l \dd N(0, I_{\theta_0}).
\]
This implies that for bowl-shaped loss functions, no regular estimator can be more accurate than those which achieve a mean zero Gaussian with the inverse Fisher information as variance.
We call estimators which achieve this, efficient.

Under regularity conditions, the Maximum Likelihood estimator is an efficient estimator.
For parametric Bayesian methods we have a similar result called the (parametric) Bernstein-von Mises theorem, see for example~\cite[Lemma 10.1 and 10.2]{vandervaartAsymptoticStatistics1998}.
This result describes the asymptotic shape of the posterior.
Under regularity conditions, the asymptotic shape will be a Gaussian distribution centred at an efficient estimator and with the inverse Fisher information as the variance.

The Bernstein-von Mises theorem is one tool that we can use to study the frequentist properties of Bayesian procedures.
By esthablishing the asymptotic shape, we can prove properties about the posterior, such as consistency, contraction rates and the validity of certain credible sets as asymptotic confidence sets.
When the asymptotic shape is a Gaussian with as mean an efficient estimator and as variance the inverse Fisher information, the posterior will be asymptotically as accurate as possible.
See for example~\cite[lemma 6.7 and 8.7]{ghosalFundamentalsNonparametricBayesian2017} and~\cite[Section 1.4.3.1]{franssenWhenSubjectiveObjective} using properties of the posterior distribution to give frequentist properties.

To study optimality of estimators in semiparametric statistics we want to use similar strategies.
In strict semiparametric models, models are index by two parameters, $\theta$ the parameter of interest and $F$ the nuisance parameter.
Because the nuisance parameter might be infinite dimensional, we can't simply take derivatives as in the euclidean setting.
One strategy is to take finite dimensional submodels that are differentiable in quadratic mean, compute the Fisher information and find the infimum.
A submodel for which this infimum is taken is called a least favourable submodel.
The information for the whole model is bounded from above by the information in the least favourable submodel.

\TODO{Efficient influence function maybe?}

Just as in the parametric case we can prove theorems that provide lowerbounds for the accuracy of semiparametric estimators.
In the same way as before, the semiparametric convolution theorem~\cite[Theorem 25.20]{vandervaartAsymptoticStatistics1998} together with Anderson's lemma reveal the best asymptotic distribution: mean zero Gaussian with the inverse efficient Fisher information as variance.
We call estimators which achieve this lowerbound efficient.

Now we want to construct estimators which are efficient.
One possible estimator is the full maximum likelihood estimator, which given a sample $X_1,\ldots, X_n$ from the distribution of $X$, maximizes the likelihood
\[
  (\q,F)\mapsto \prodin \int p_\q(X_i\given z)\,dF(z). 
\]
These estimators were shown to be consistent in some generality in~\cite{kieferConsistencyMaximumLikelihood1956}.
For a small number of special models the $\q$-component of the maximum likelihood estimator is known to be asymptotically normal and efficient from~\cite{vandervaartEstimatingRealParameter1988,murphyLikelihoodInferenceErrorsinVariables1996,vandervaartEfficientMaximumLikelihood1996}. 

A Bayesian alternative is to equip $F$ with a species sampling prior, and, independetly $\theta$ with a smooth prior.
Two common choices for a mixture prior would be the Dirichlet process prior or a finite discrete prior with a random number of components.
These two choices are the priors we will study in our examples.

The Dirichlet process is a stochastic process characterised by two parameters, the prior precision $M$ and the center measure $G$.
Then a random variable $F$ is said to be Dirichlet process distributed if for any partition $A_1, \dots A_k$
\[
    (F(A_1),\dots, F(A_k)) \sim \textrm{Dir}\left(k; MG(A_1),\dots, MG(A_k)\right).
\]

As an example of a finitely discrete prior with a random number of components, pick $\lambda, \sigma > 0$ and $G$ a probability distribution.
Then we draw $K \sim \textrm{Geom}(\lambda)$, and given $K$ draw $Z_1, \dots, Z_K \overset{\textrm{i.i.d.}}\sim G$, $W \sim \textrm{Dir}(K; \sigma,\dots, \sigma)$.
Then 
\[
    F = \sum_{i = 1}^K W_i \delta_{Z_i}
\]
We will give more details on these priors in \cref{sec:priors}. 
Here we will also recall the facts that are needed for the purpose of this paper.

More generally, a species sampling process can be defined using the exchangeable partition probability function (EPPF) and a center measure $G$.
There are many more examples of species sampling process priors, for example the Pitman-Yor processes, Gibbs processes or Poisson-Kingman processes.
For more details, see~\cite[Chapter 14]{ghosalFundamentalsNonparametricBayesian2017}.

To show the asymptotical optimality of the Bayesian methodology, we prove a Bernstein-von Mises theorem for $\theta$.
In~\cite{castilloSemiparametricBernsteinMises2012}, Castillo derived conditions for the Bernstein-von Mises theorem to hold for specific Models and Gaussian process priors.
This work has later been extended by~\cite{bickelSemiparametricBernsteinMises2012,castilloBernsteinvonMisesPhenomenon2014,castilloBernsteinMisesTheorem2015,raySemiparametricBayesianCausal2020}.
In these works, the authors prove the Bernstein-von Mises result under two assumptions.
The first of these assumptions is a locally asymptotically normal (LAN) expansion of the likelihood in a perturbation.
This condition closely resembles the assumptions needed to make the MLE efficient.
The second of these assumptions is a change of measure condition.
This condition roughly states that the prior and the perturbation interact nicely.

Not only was efficiency of the Bayesian models an open question, consistency, or the ability to concentrate all mass near the true parameter was also unknown.
In \cref{sec:consistency} we provide two tools to show that the posterior distribution is consistent in mixture models. 
The first is based on the seminal works by Kiefer and Wolfowitz~\cite{kieferConsistencyMaximumLikelihood1956} and Schwartz~\cite{schwartzBayesProcedures1965} (see also~\cite[Lemma 6.16 and 6.17]{ghosalFundamentalsNonparametricBayesian2017}).
The second technique uses the Glivenko-Cantelli theorem and Schwartz's theorem again.

Consistency allows us to localise our assumptions to a neighbourhood of the truth.
This allows us to tackle the LAN expansion and the change of measure condition locally.
In \cref{sec:semiparBvM} we formulate a precise theorem including the assumption on the LAN expansion and the change of measure.

To verify the LAN expansion we provide a lemma in terms of Donsker conditions in \cref{sec:LAN}.
There are advantages and disadvantages to this approach.
Donsker conditions are technical conditions that can require work to verify.
However, since the asymptotic efficiency for the MLE also relies on Donsker conditions, this work has often already been done in earlier papers.

Before this work, the main issue lay with verifying the second condition.
We had no tools to verify this for mixture models.
This is a fundamental gap in our understanding of the behaviour of Bayesian methods in these popular models.
In \cref{sec:changeofmeasure} we provide the tools to verify this condition. 

Finally we verify these assumptions for two semiparametric mixture models.
In \cref{sec:frailty} we study the frailty model, while in \cref{sec:ErrorsInVars} we study the errors in variables model.


